Paving the Way for Consensus: Convergence of Block Gossip Algorithms

Gossip protocols are popular methods for average consensus problems in distributed computing. We prove new convergence guarantees for a variety of such protocols, including path, clique, and synchronous pairwise gossip. These arise by exploiting the connection between these protocols and the block randomized Kaczmarz method for solving linear systems. Moreover, we extend existing convergence results for block randomized Kaczmarz to allow for a more general choice of blocks, rank-deficient systems, and provide a tighter convergence rate guarantee. We furthermore apply this analysis to inconsistent consensus models and obtain similar guarantees. An extensive empirical analysis of these methods is provided for a variety of synthetic networks.

==> figs/p02_all_methods <==
<?xml version="1.0" encoding="utf-8" standalone="no"?>
<!DOCTYPE svg PUBLIC "-//W3C//DTD SVG 1.1//EN"
  "http://www.w3.org/Graphics/SVG/1.1/DTD/svg11.dtd">
<svg height="432pt" version="1.1" viewBox="0 0 576 432" width="576pt" xmlns="http://www.w3.org/2000/svg" xmlns:xlink="http://www.w3.org/1999/xlink">
 <metadata>
  <rdf:RDF xmlns:cc="http://creativecommons.org/ns#" xmlns:dc="http://purl.org/dc/elements/1.1/" xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#">
   <cc:Work>
    <dc:type rdf:resource="http://purl.org/dc/dcmitype/StillImage"/>
    <dc:date>2021-10-19T15:47:49.912705</dc:date>
    <dc:format>image/svg+xml</dc:format>
    <dc:creator>
     <cc:Agent>
      <dc:title>Matplotlib v3.4.2, https://matplotlib.org/</dc:title>
     </cc:Agent>
    </dc:creator>
   </cc:Work>
  </rdf:RDF>
 </metadata>
 <defs>
  <style type="text/css">*{stroke-linecap:butt;stroke-linejoin:round;}</style>
 </defs>
 <g id="figure_1">
  <g id="patch_1">
   <path d="M 0 432 
L 576 432 
L 576 0 
L 0 0 
z
" style="fill:none;"/>
  </g>
  <g id="axes_1">
   <g id="patch_2">
    <path d="M 72 378 
L 518.4 378 
L 518.4 51.84 
L 72 51.84 
z
" style="fill:#ffffff;"/>
   </g>
   <g id="matplotlib.axis_1">
    <g id="xtick_1">
     <g id="line2d_1">
      <defs>
       <path d="M 0 0 
L 0 3.5 
" id="m4edf43f6d4" style="stroke:#000000;stroke-width:0.8;"/>
      </defs>
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="92.290909" xlink:href="#m4edf43f6d4" y="378"/>
      </g>
     </g>
     <g id="text_1">
      <!-- 0 -->
      <g transform="translate(87.519034 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 2034 4250 
Q 1547 4250 1301 3770 
Q 1056 3291 1056 2328 
Q 1056 1369 1301 889 
Q 1547 409 2034 409 
Q 2525 409 2770 889 
Q 3016 1369 3016 2328 
Q 3016 3291 2770 3770 
Q 2525 4250 2034 4250 
z
M 2034 4750 
Q 2819 4750 3233 4129 
Q 3647 3509 3647 2328 
Q 3647 1150 3233 529 
Q 2819 -91 2034 -91 
Q 1250 -91 836 529 
Q 422 1150 422 2328 
Q 422 3509 836 4129 
Q 1250 4750 2034 4750 
z
" id="DejaVuSans-30" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_2">
     <g id="line2d_2">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="143.273093" xlink:href="#m4edf43f6d4" y="378"/>
      </g>
     </g>
     <g id="text_2">
      <!-- 25 -->
      <g transform="translate(133.729343 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 1228 531 
L 3431 531 
L 3431 0 
L 469 0 
L 469 531 
Q 828 903 1448 1529 
Q 2069 2156 2228 2338 
Q 2531 2678 2651 2914 
Q 2772 3150 2772 3378 
Q 2772 3750 2511 3984 
Q 2250 4219 1831 4219 
Q 1534 4219 1204 4116 
Q 875 4013 500 3803 
L 500 4441 
Q 881 4594 1212 4672 
Q 1544 4750 1819 4750 
Q 2544 4750 2975 4387 
Q 3406 4025 3406 3419 
Q 3406 3131 3298 2873 
Q 3191 2616 2906 2266 
Q 2828 2175 2409 1742 
Q 1991 1309 1228 531 
z
" id="DejaVuSans-32" transform="scale(0.015625)"/>
        <path d="M 691 4666 
L 3169 4666 
L 3169 4134 
L 1269 4134 
L 1269 2991 
Q 1406 3038 1543 3061 
Q 1681 3084 1819 3084 
Q 2600 3084 3056 2656 
Q 3513 2228 3513 1497 
Q 3513 744 3044 326 
Q 2575 -91 1722 -91 
Q 1428 -91 1123 -41 
Q 819 9 494 109 
L 494 744 
Q 775 591 1075 516 
Q 1375 441 1709 441 
Q 2250 441 2565 725 
Q 2881 1009 2881 1497 
Q 2881 1984 2565 2268 
Q 2250 2553 1709 2553 
Q 1456 2553 1204 2497 
Q 953 2441 691 2322 
L 691 4666 
z
" id="DejaVuSans-35" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-32"/>
       <use x="63.623047" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_3">
     <g id="line2d_3">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="194.255276" xlink:href="#m4edf43f6d4" y="378"/>
      </g>
     </g>
     <g id="text_3">
      <!-- 50 -->
      <g transform="translate(184.711526 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-35"/>
       <use x="63.623047" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_4">
     <g id="line2d_4">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="245.23746" xlink:href="#m4edf43f6d4" y="378"/>
      </g>
     </g>
     <g id="text_4">
      <!-- 75 -->
      <g transform="translate(235.69371 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 525 4666 
L 3525 4666 
L 3525 4397 
L 1831 0 
L 1172 0 
L 2766 4134 
L 525 4134 
L 525 4666 
z
" id="DejaVuSans-37" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-37"/>
       <use x="63.623047" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_5">
     <g id="line2d_5">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="296.219644" xlink:href="#m4edf43f6d4" y="378"/>
      </g>
     </g>
     <g id="text_5">
      <!-- 100 -->
      <g transform="translate(281.904019 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 794 531 
L 1825 531 
L 1825 4091 
L 703 3866 
L 703 4441 
L 1819 4666 
L 2450 4666 
L 2450 531 
L 3481 531 
L 3481 0 
L 794 0 
L 794 531 
z
" id="DejaVuSans-31" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-30"/>
       <use x="127.246094" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_6">
     <g id="line2d_6">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="347.201827" xlink:href="#m4edf43f6d4" y="378"/>
      </g>
     </g>
     <g id="text_6">
      <!-- 125 -->
      <g transform="translate(332.886202 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-32"/>
       <use x="127.246094" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_7">
     <g id="line2d_7">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="398.184011" xlink:href="#m4edf43f6d4" y="378"/>
      </g>
     </g>
     <g id="text_7">
      <!-- 150 -->
      <g transform="translate(383.868386 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-35"/>
       <use x="127.246094" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_8">
     <g id="line2d_8">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="449.166195" xlink:href="#m4edf43f6d4" y="378"/>
      </g>
     </g>
     <g id="text_8">
      <!-- 175 -->
      <g transform="translate(434.85057 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-37"/>
       <use x="127.246094" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_9">
     <g id="line2d_9">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="500.148378" xlink:href="#m4edf43f6d4" y="378"/>
      </g>
     </g>
     <g id="text_9">
      <!-- 200 -->
      <g transform="translate(485.832753 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-32"/>
       <use x="63.623047" xlink:href="#DejaVuSans-30"/>
       <use x="127.246094" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="text_10">
     <!-- Iteration number, $k$ -->
     <g transform="translate(222.6 414.914844)scale(0.15 -0.15)">
      <defs>
       <path d="M 628 4666 
L 1259 4666 
L 1259 0 
L 628 0 
L 628 4666 
z
" id="DejaVuSans-49" transform="scale(0.015625)"/>
       <path d="M 1172 4494 
L 1172 3500 
L 2356 3500 
L 2356 3053 
L 1172 3053 
L 1172 1153 
Q 1172 725 1289 603 
Q 1406 481 1766 481 
L 2356 481 
L 2356 0 
L 1766 0 
Q 1100 0 847 248 
Q 594 497 594 1153 
L 594 3053 
L 172 3053 
L 172 3500 
L 594 3500 
L 594 4494 
L 1172 4494 
z
" id="DejaVuSans-74" transform="scale(0.015625)"/>
       <path d="M 3597 1894 
L 3597 1613 
L 953 1613 
Q 991 1019 1311 708 
Q 1631 397 2203 397 
Q 2534 397 2845 478 
Q 3156 559 3463 722 
L 3463 178 
Q 3153 47 2828 -22 
Q 2503 -91 2169 -91 
Q 1331 -91 842 396 
Q 353 884 353 1716 
Q 353 2575 817 3079 
Q 1281 3584 2069 3584 
Q 2775 3584 3186 3129 
Q 3597 2675 3597 1894 
z
M 3022 2063 
Q 3016 2534 2758 2815 
Q 2500 3097 2075 3097 
Q 1594 3097 1305 2825 
Q 1016 2553 972 2059 
L 3022 2063 
z
" id="DejaVuSans-65" transform="scale(0.015625)"/>
       <path d="M 2631 2963 
Q 2534 3019 2420 3045 
Q 2306 3072 2169 3072 
Q 1681 3072 1420 2755 
Q 1159 2438 1159 1844 
L 1159 0 
L 581 0 
L 581 3500 
L 1159 3500 
L 1159 2956 
Q 1341 3275 1631 3429 
Q 1922 3584 2338 3584 
Q 2397 3584 2469 3576 
Q 2541 3569 2628 3553 
L 2631 2963 
z
" id="DejaVuSans-72" transform="scale(0.015625)"/>
       <path d="M 2194 1759 
Q 1497 1759 1228 1600 
Q 959 1441 959 1056 
Q 959 750 1161 570 
Q 1363 391 1709 391 
Q 2188 391 2477 730 
Q 2766 1069 2766 1631 
L 2766 1759 
L 2194 1759 
z
M 3341 1997 
L 3341 0 
L 2766 0 
L 2766 531 
Q 2569 213 2275 61 
Q 1981 -91 1556 -91 
Q 1019 -91 701 211 
Q 384 513 384 1019 
Q 384 1609 779 1909 
Q 1175 2209 1959 2209 
L 2766 2209 
L 2766 2266 
Q 2766 2663 2505 2880 
Q 2244 3097 1772 3097 
Q 1472 3097 1187 3025 
Q 903 2953 641 2809 
L 641 3341 
Q 956 3463 1253 3523 
Q 1550 3584 1831 3584 
Q 2591 3584 2966 3190 
Q 3341 2797 3341 1997 
z
" id="DejaVuSans-61" transform="scale(0.015625)"/>
       <path d="M 603 3500 
L 1178 3500 
L 1178 0 
L 603 0 
L 603 3500 
z
M 603 4863 
L 1178 4863 
L 1178 4134 
L 603 4134 
L 603 4863 
z
" id="DejaVuSans-69" transform="scale(0.015625)"/>
       <path d="M 1959 3097 
Q 1497 3097 1228 2736 
Q 959 2375 959 1747 
Q 959 1119 1226 758 
Q 1494 397 1959 397 
Q 2419 397 2687 759 
Q 2956 1122 2956 1747 
Q 2956 2369 2687 2733 
Q 2419 3097 1959 3097 
z
M 1959 3584 
Q 2709 3584 3137 3096 
Q 3566 2609 3566 1747 
Q 3566 888 3137 398 
Q 2709 -91 1959 -91 
Q 1206 -91 779 398 
Q 353 888 353 1747 
Q 353 2609 779 3096 
Q 1206 3584 1959 3584 
z
" id="DejaVuSans-6f" transform="scale(0.015625)"/>
       <path d="M 3513 2113 
L 3513 0 
L 2938 0 
L 2938 2094 
Q 2938 2591 2744 2837 
Q 2550 3084 2163 3084 
Q 1697 3084 1428 2787 
Q 1159 2491 1159 1978 
L 1159 0 
L 581 0 
L 581 3500 
L 1159 3500 
L 1159 2956 
Q 1366 3272 1645 3428 
Q 1925 3584 2291 3584 
Q 2894 3584 3203 3211 
Q 3513 2838 3513 2113 
z
" id="DejaVuSans-6e" transform="scale(0.015625)"/>
       <path id="DejaVuSans-20" transform="scale(0.015625)"/>
       <path d="M 544 1381 
L 544 3500 
L 1119 3500 
L 1119 1403 
Q 1119 906 1312 657 
Q 1506 409 1894 409 
Q 2359 409 2629 706 
Q 2900 1003 2900 1516 
L 2900 3500 
L 3475 3500 
L 3475 0 
L 2900 0 
L 2900 538 
Q 2691 219 2414 64 
Q 2138 -91 1772 -91 
Q 1169 -91 856 284 
Q 544 659 544 1381 
z
M 1991 3584 
L 1991 3584 
z
" id="DejaVuSans-75" transform="scale(0.015625)"/>
       <path d="M 3328 2828 
Q 3544 3216 3844 3400 
Q 4144 3584 4550 3584 
Q 5097 3584 5394 3201 
Q 5691 2819 5691 2113 
L 5691 0 
L 5113 0 
L 5113 2094 
Q 5113 2597 4934 2840 
Q 4756 3084 4391 3084 
Q 3944 3084 3684 2787 
Q 3425 2491 3425 1978 
L 3425 0 
L 2847 0 
L 2847 2094 
Q 2847 2600 2669 2842 
Q 2491 3084 2119 3084 
Q 1678 3084 1418 2786 
Q 1159 2488 1159 1978 
L 1159 0 
L 581 0 
L 581 3500 
L 1159 3500 
L 1159 2956 
Q 1356 3278 1631 3431 
Q 1906 3584 2284 3584 
Q 2666 3584 2933 3390 
Q 3200 3197 3328 2828 
z
" id="DejaVuSans-6d" transform="scale(0.015625)"/>
       <path d="M 3116 1747 
Q 3116 2381 2855 2742 
Q 2594 3103 2138 3103 
Q 1681 3103 1420 2742 
Q 1159 2381 1159 1747 
Q 1159 1113 1420 752 
Q 1681 391 2138 391 
Q 2594 391 2855 752 
Q 3116 1113 3116 1747 
z
M 1159 2969 
Q 1341 3281 1617 3432 
Q 1894 3584 2278 3584 
Q 2916 3584 3314 3078 
Q 3713 2572 3713 1747 
Q 3713 922 3314 415 
Q 2916 -91 2278 -91 
Q 1894 -91 1617 61 
Q 1341 213 1159 525 
L 1159 0 
L 581 0 
L 581 4863 
L 1159 4863 
L 1159 2969 
z
" id="DejaVuSans-62" transform="scale(0.015625)"/>
       <path d="M 750 794 
L 1409 794 
L 1409 256 
L 897 -744 
L 494 -744 
L 750 256 
L 750 794 
z
" id="DejaVuSans-2c" transform="scale(0.015625)"/>
       <path d="M 1172 4863 
L 1747 4863 
L 1197 2028 
L 3169 3500 
L 3916 3500 
L 1716 1825 
L 3322 0 
L 2625 0 
L 1131 1709 
L 800 0 
L 225 0 
L 1172 4863 
z
" id="DejaVuSans-Oblique-6b" transform="scale(0.015625)"/>
      </defs>
      <use transform="translate(0 0.015625)" xlink:href="#DejaVuSans-49"/>
      <use transform="translate(29.492188 0.015625)" xlink:href="#DejaVuSans-74"/>
      <use transform="translate(68.701172 0.015625)" xlink:href="#DejaVuSans-65"/>
      <use transform="translate(130.224609 0.015625)" xlink:href="#DejaVuSans-72"/>
      <use transform="translate(171.337891 0.015625)" xlink:href="#DejaVuSans-61"/>
      <use transform="translate(232.617188 0.015625)" xlink:href="#DejaVuSans-74"/>
      <use transform="translate(271.826172 0.015625)" xlink:href="#DejaVuSans-69"/>
      <use transform="translate(299.609375 0.015625)" xlink:href="#DejaVuSans-6f"/>
      <use transform="translate(360.791016 0.015625)" xlink:href="#DejaVuSans-6e"/>
      <use transform="translate(424.169922 0.015625)" xlink:href="#DejaVuSans-20"/>
      <use transform="translate(455.957031 0.015625)" xlink:href="#DejaVuSans-6e"/>
      <use transform="translate(519.335938 0.015625)" xlink:href="#DejaVuSans-75"/>
      <use transform="translate(582.714844 0.015625)" xlink:href="#DejaVuSans-6d"/>
      <use transform="translate(680.126953 0.015625)" xlink:href="#DejaVuSans-62"/>
      <use transform="translate(743.603516 0.015625)" xlink:href="#DejaVuSans-65"/>
      <use transform="translate(805.126953 0.015625)" xlink:href="#DejaVuSans-72"/>
      <use transform="translate(846.240234 0.015625)" xlink:href="#DejaVuSans-2c"/>
      <use transform="translate(878.027344 0.015625)" xlink:href="#DejaVuSans-20"/>
      <use transform="translate(909.814453 0.015625)" xlink:href="#DejaVuSans-Oblique-6b"/>
     </g>
    </g>
   </g>
   <g id="matplotlib.axis_2">
    <g id="ytick_1">
     <g id="line2d_10">
      <defs>
       <path d="M 0 0 
L -3.5 0 
" id="m65750edd41" style="stroke:#000000;stroke-width:0.8;"/>
      </defs>
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m65750edd41" y="344.060607"/>
      </g>
     </g>
     <g id="text_11">
      <!-- $\mathdefault{10^{-28}}$ -->
      <g transform="translate(23.15 349.759435)scale(0.15 -0.15)">
       <defs>
        <path d="M 678 2272 
L 4684 2272 
L 4684 1741 
L 678 1741 
L 678 2272 
z
" id="DejaVuSans-2212" transform="scale(0.015625)"/>
        <path d="M 2034 2216 
Q 1584 2216 1326 1975 
Q 1069 1734 1069 1313 
Q 1069 891 1326 650 
Q 1584 409 2034 409 
Q 2484 409 2743 651 
Q 3003 894 3003 1313 
Q 3003 1734 2745 1975 
Q 2488 2216 2034 2216 
z
M 1403 2484 
Q 997 2584 770 2862 
Q 544 3141 544 3541 
Q 544 4100 942 4425 
Q 1341 4750 2034 4750 
Q 2731 4750 3128 4425 
Q 3525 4100 3525 3541 
Q 3525 3141 3298 2862 
Q 3072 2584 2669 2484 
Q 3125 2378 3379 2068 
Q 3634 1759 3634 1313 
Q 3634 634 3220 271 
Q 2806 -91 2034 -91 
Q 1263 -91 848 271 
Q 434 634 434 1313 
Q 434 1759 690 2068 
Q 947 2378 1403 2484 
z
M 1172 3481 
Q 1172 3119 1398 2916 
Q 1625 2713 2034 2713 
Q 2441 2713 2670 2916 
Q 2900 3119 2900 3481 
Q 2900 3844 2670 4047 
Q 2441 4250 2034 4250 
Q 1625 4250 1398 4047 
Q 1172 3844 1172 3481 
z
" id="DejaVuSans-38" transform="scale(0.015625)"/>
       </defs>
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-38"/>
      </g>
     </g>
    </g>
    <g id="ytick_2">
     <g id="line2d_11">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m65750edd41" y="306.052274"/>
      </g>
     </g>
     <g id="text_12">
      <!-- $\mathdefault{10^{-24}}$ -->
      <g transform="translate(23.15 311.751102)scale(0.15 -0.15)">
       <defs>
        <path d="M 2419 4116 
L 825 1625 
L 2419 1625 
L 2419 4116 
z
M 2253 4666 
L 3047 4666 
L 3047 1625 
L 3713 1625 
L 3713 1100 
L 3047 1100 
L 3047 0 
L 2419 0 
L 2419 1100 
L 313 1100 
L 313 1709 
L 2253 4666 
z
" id="DejaVuSans-34" transform="scale(0.015625)"/>
       </defs>
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-34"/>
      </g>
     </g>
    </g>
    <g id="ytick_3">
     <g id="line2d_12">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m65750edd41" y="268.043941"/>
      </g>
     </g>
     <g id="text_13">
      <!-- $\mathdefault{10^{-20}}$ -->
      <g transform="translate(23.15 273.742769)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="ytick_4">
     <g id="line2d_13">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m65750edd41" y="230.035608"/>
      </g>
     </g>
     <g id="text_14">
      <!-- $\mathdefault{10^{-16}}$ -->
      <g transform="translate(23.15 235.734436)scale(0.15 -0.15)">
       <defs>
        <path d="M 2113 2584 
Q 1688 2584 1439 2293 
Q 1191 2003 1191 1497 
Q 1191 994 1439 701 
Q 1688 409 2113 409 
Q 2538 409 2786 701 
Q 3034 994 3034 1497 
Q 3034 2003 2786 2293 
Q 2538 2584 2113 2584 
z
M 3366 4563 
L 3366 3988 
Q 3128 4100 2886 4159 
Q 2644 4219 2406 4219 
Q 1781 4219 1451 3797 
Q 1122 3375 1075 2522 
Q 1259 2794 1537 2939 
Q 1816 3084 2150 3084 
Q 2853 3084 3261 2657 
Q 3669 2231 3669 1497 
Q 3669 778 3244 343 
Q 2819 -91 2113 -91 
Q 1303 -91 875 529 
Q 447 1150 447 2328 
Q 447 3434 972 4092 
Q 1497 4750 2381 4750 
Q 2619 4750 2861 4703 
Q 3103 4656 3366 4563 
z
" id="DejaVuSans-36" transform="scale(0.015625)"/>
       </defs>
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-36"/>
      </g>
     </g>
    </g>
    <g id="ytick_5">
     <g id="line2d_14">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m65750edd41" y="192.027275"/>
      </g>
     </g>
     <g id="text_15">
      <!-- $\mathdefault{10^{-12}}$ -->
      <g transform="translate(23.15 197.726103)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
      </g>
     </g>
    </g>
    <g id="ytick_6">
     <g id="line2d_15">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m65750edd41" y="154.018942"/>
      </g>
     </g>
     <g id="text_16">
      <!-- $\mathdefault{10^{-8}}$ -->
      <g transform="translate(29.75 159.71777)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-38"/>
      </g>
     </g>
    </g>
    <g id="ytick_7">
     <g id="line2d_16">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m65750edd41" y="116.010609"/>
      </g>
     </g>
     <g id="text_17">
      <!-- $\mathdefault{10^{-4}}$ -->
      <g transform="translate(29.75 121.709437)scale(0.15 -0.15)">
       <use transform="translate(0 0.684375)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.684375)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 38.965625)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 38.965625)scale(0.7)" xlink:href="#DejaVuSans-34"/>
      </g>
     </g>
    </g>
    <g id="ytick_8">
     <g id="line2d_17">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m65750edd41" y="78.002275"/>
      </g>
     </g>
     <g id="text_18">
      <!-- $\mathdefault{10^{0}}$ -->
      <g transform="translate(38.6 83.701104)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="text_19">
     <!-- $||c_k-c*||^2$ -->
     <g transform="translate(15.55 256.02)rotate(-90)scale(0.15 -0.15)">
      <defs>
       <path d="M 1344 4891 
L 1344 -1509 
L 813 -1509 
L 813 4891 
L 1344 4891 
z
" id="DejaVuSans-7c" transform="scale(0.015625)"/>
       <path d="M 3431 3366 
L 3316 2797 
Q 3109 2947 2876 3022 
Q 2644 3097 2394 3097 
Q 2119 3097 1870 3000 
Q 1622 2903 1453 2725 
Q 1184 2453 1037 2087 
Q 891 1722 891 1331 
Q 891 859 1127 628 
Q 1363 397 1844 397 
Q 2081 397 2348 469 
Q 2616 541 2906 684 
L 2797 116 
Q 2547 13 2283 -39 
Q 2019 -91 1741 -91 
Q 1044 -91 669 257 
Q 294 606 294 1253 
Q 294 1797 489 2255 
Q 684 2713 1069 3078 
Q 1331 3328 1684 3456 
Q 2038 3584 2456 3584 
Q 2700 3584 2940 3529 
Q 3181 3475 3431 3366 
z
" id="DejaVuSans-Oblique-63" transform="scale(0.015625)"/>
       <path d="M 3009 3897 
L 1888 3291 
L 3009 2681 
L 2828 2375 
L 1778 3009 
L 1778 1831 
L 1422 1831 
L 1422 3009 
L 372 2375 
L 191 2681 
L 1313 3291 
L 191 3897 
L 372 4206 
L 1422 3572 
L 1422 4750 
L 1778 4750 
L 1778 3572 
L 2828 4206 
L 3009 3897 
z
" id="DejaVuSans-2a" transform="scale(0.015625)"/>
      </defs>
      <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(33.691406 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(67.382812 0.765625)" xlink:href="#DejaVuSans-Oblique-63"/>
      <use transform="translate(122.363281 -15.640625)scale(0.7)" xlink:href="#DejaVuSans-Oblique-6b"/>
      <use transform="translate(185.117188 0.765625)" xlink:href="#DejaVuSans-2212"/>
      <use transform="translate(288.388672 0.765625)" xlink:href="#DejaVuSans-Oblique-63"/>
      <use transform="translate(362.851562 0.765625)" xlink:href="#DejaVuSans-2a"/>
      <use transform="translate(432.333984 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(466.025391 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(500.673828 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
     </g>
    </g>
   </g>
   <g id="line2d_18">
    <path clip-path="url(#p163a1be3ee)" d="M 92.290909 66.671164 
L 102.487346 66.813048 
L 114.72307 66.836498 
L 116.762357 66.974193 
L 120.840932 67.065394 
L 124.919507 67.14306 
L 147.351667 67.566011 
L 151.430242 67.677976 
L 179.980265 68.143365 
L 188.137414 68.34113 
L 200.373138 68.527373 
L 220.766012 69.144341 
L 228.923161 69.315424 
L 247.276747 69.519788 
L 251.355322 69.550441 
L 253.394609 69.731501 
L 257.473184 69.779467 
L 259.512471 69.959929 
L 261.551759 69.96342 
L 263.591046 70.081677 
L 265.630333 70.084244 
L 269.708908 70.279024 
L 275.82677 70.396407 
L 294.180356 70.638084 
L 312.533942 70.696844 
L 316.612517 70.804579 
L 326.808954 70.841055 
L 330.887529 70.964536 
L 334.966103 71.011186 
L 337.005391 71.173801 
L 377.791138 71.541196 
L 379.830425 71.663263 
L 390.026862 71.733734 
L 396.144724 71.827362 
L 398.184011 71.842379 
L 400.223298 72.101483 
L 432.851896 72.367495 
L 436.930471 72.449026 
L 451.205482 72.557132 
L 498.109091 73.013721 
L 498.109091 73.013721 
" style="fill:none;stroke:#0000ff;stroke-linecap:square;stroke-width:3;"/>
   </g>
   <g id="line2d_19">
    <path clip-path="url(#p163a1be3ee)" d="M 92.290909 68.859018 
L 94.330196 70.93141 
L 96.369484 72.008096 
L 98.408771 74.106993 
L 100.448058 78.206564 
L 102.487346 78.920955 
L 106.565921 82.761266 
L 108.605208 83.031595 
L 110.644495 84.544572 
L 112.683783 86.979769 
L 114.72307 88.873273 
L 116.762357 90.483344 
L 118.801645 92.767607 
L 120.840932 95.547537 
L 122.880219 95.793331 
L 124.919507 96.263087 
L 126.958794 98.342613 
L 128.998081 100.884111 
L 133.076656 102.590588 
L 135.115943 104.295413 
L 137.155231 106.161691 
L 139.194518 106.375987 
L 143.273093 111.460498 
L 145.31238 114.031805 
L 147.351667 116.795612 
L 149.390955 117.668442 
L 153.469529 122.632522 
L 155.508817 124.570205 
L 157.548104 125.429324 
L 159.587392 128.194506 
L 163.665966 132.424342 
L 165.705254 133.390508 
L 167.744541 136.458003 
L 169.783828 136.64842 
L 173.862403 137.483943 
L 175.90169 140.11856 
L 177.940978 142.021184 
L 179.980265 144.266033 
L 182.019552 147.614601 
L 184.05884 147.694459 
L 186.098127 148.969947 
L 188.137414 151.000834 
L 190.176702 152.488622 
L 192.215989 154.252261 
L 194.255276 156.916395 
L 196.294564 159.365193 
L 198.333851 160.593482 
L 200.373138 162.860598 
L 202.412426 163.399691 
L 204.451713 165.867255 
L 206.491 167.937769 
L 210.569575 172.850971 
L 212.608862 175.094134 
L 214.64815 175.521573 
L 216.687437 176.122375 
L 218.726725 177.841733 
L 220.766012 179.793307 
L 222.805299 181.246184 
L 226.883874 186.539294 
L 228.923161 187.395419 
L 230.962449 190.055933 
L 233.001736 191.211292 
L 235.041023 194.299466 
L 237.080311 195.780392 
L 239.119598 197.55963 
L 241.158885 198.736934 
L 243.198173 198.954395 
L 247.276747 204.697454 
L 249.316035 207.567638 
L 251.355322 208.757853 
L 253.394609 210.317562 
L 255.433897 212.987765 
L 259.512471 214.402387 
L 261.551759 216.436478 
L 263.591046 217.583138 
L 265.630333 219.181754 
L 267.669621 222.260221 
L 269.708908 223.159043 
L 271.748196 225.934464 
L 273.787483 227.95089 
L 275.82677 230.542361 
L 277.866058 232.760649 
L 279.905345 233.528301 
L 281.944632 235.84614 
L 283.98392 237.897234 
L 286.023207 239.042491 
L 288.062494 239.764481 
L 290.101782 240.858909 
L 292.141069 241.381596 
L 294.180356 244.306482 
L 296.219644 245.033417 
L 298.258931 247.193711 
L 300.298218 247.583545 
L 302.337506 247.858491 
L 304.376793 250.721253 
L 306.41608 253.130761 
L 308.455368 255.216625 
L 310.494655 256.166746 
L 312.533942 258.6526 
L 314.57323 260.445647 
L 316.612517 263.259395 
L 318.651804 265.676682 
L 320.691092 268.731948 
L 324.769667 272.797544 
L 326.808954 275.878247 
L 328.848241 277.624096 
L 330.887529 280.152467 
L 332.926816 281.359751 
L 334.966103 283.133763 
L 337.005391 285.464708 
L 339.044678 286.361068 
L 341.083965 287.433721 
L 343.123253 290.440338 
L 345.16254 292.984039 
L 347.201827 293.838672 
L 351.280402 294.978064 
L 353.319689 297.658117 
L 355.358977 298.698049 
L 357.398264 300.12234 
L 359.437551 300.686227 
L 363.516126 306.790595 
L 365.555413 309.608675 
L 367.594701 310.44589 
L 369.633988 313.14604 
L 371.673275 314.913597 
L 373.712563 316.41806 
L 377.791138 319.060656 
L 379.830425 321.221273 
L 381.869712 323.568177 
L 383.909 325.307355 
L 385.948287 325.383271 
L 387.987574 327.173953 
L 390.026862 328.698287 
L 392.066149 330.87125 
L 394.105436 331.562968 
L 396.144724 333.064632 
L 400.223298 338.524539 
L 402.262586 339.717972 
L 404.301873 341.987092 
L 406.34116 343.882881 
L 408.380448 345.363133 
L 412.459022 351.22369 
L 416.537597 354.990546 
L 418.576884 355.728579 
L 420.616172 358.027214 
L 422.655459 359.239478 
L 424.694746 359.403747 
L 426.734034 359.707957 
L 428.773321 361.589304 
L 430.812608 362.327486 
L 432.851896 362.501267 
L 434.891183 362.160727 
L 436.930471 362.636581 
L 438.969758 362.921294 
L 441.009045 363.071373 
L 449.166195 363.071373 
L 451.205482 362.824191 
L 453.244769 362.72932 
L 455.284057 363.122637 
L 457.323344 362.243264 
L 465.480493 362.160727 
L 467.519781 361.589304 
L 469.559068 361.449403 
L 471.598355 361.518761 
L 475.67693 361.280943 
L 481.794792 360.501136 
L 498.109091 360.135239 
L 498.109091 360.135239 
" style="fill:none;stroke:#008000;stroke-dasharray:11.1,4.8;stroke-dashoffset:0;stroke-width:3;"/>
   </g>
   <g id="line2d_20">
    <path clip-path="url(#p163a1be3ee)" d="M 92.290909 66.665455 
L 98.408771 67.136538 
L 106.565921 67.809687 
L 110.644495 68.113569 
L 112.683783 68.366547 
L 116.762357 68.538036 
L 118.801645 68.828425 
L 126.958794 69.38633 
L 131.037369 69.814629 
L 133.076656 70.323126 
L 137.155231 70.804905 
L 139.194518 70.883488 
L 145.31238 71.534188 
L 147.351667 71.559774 
L 151.430242 71.9385 
L 153.469529 72.053024 
L 159.587392 72.831851 
L 161.626679 72.847338 
L 163.665966 73.581309 
L 165.705254 73.951573 
L 167.744541 74.170801 
L 169.783828 74.715727 
L 198.333851 75.552688 
L 200.373138 75.941076 
L 206.491 76.179774 
L 210.569575 76.253625 
L 212.608862 76.706568 
L 214.64815 76.9529 
L 218.726725 77.067685 
L 222.805299 78.42577 
L 228.923161 78.489819 
L 230.962449 78.92132 
L 245.23746 79.173109 
L 251.355322 79.231233 
L 253.394609 81.34514 
L 255.433897 81.359682 
L 257.473184 81.523169 
L 265.630333 81.802299 
L 267.669621 81.920856 
L 269.708908 82.453597 
L 277.866058 82.721336 
L 279.905345 82.898077 
L 281.944632 87.288952 
L 283.98392 87.424215 
L 286.023207 87.733409 
L 288.062494 87.804511 
L 292.141069 88.193558 
L 294.180356 88.394378 
L 304.376793 88.625346 
L 306.41608 88.756967 
L 308.455368 89.438391 
L 310.494655 89.460909 
L 312.533942 89.796617 
L 314.57323 90.570235 
L 316.612517 90.804703 
L 318.651804 91.358241 
L 330.887529 92.205318 
L 332.926816 92.890589 
L 334.966103 92.945092 
L 337.005391 93.393253 
L 343.123253 93.622415 
L 365.555413 93.886936 
L 367.594701 94.17897 
L 371.673275 94.205389 
L 373.712563 94.622464 
L 375.75185 94.642429 
L 377.791138 95.12372 
L 394.105436 95.341718 
L 400.223298 95.470605 
L 404.301873 95.483836 
L 406.34116 95.687398 
L 412.459022 95.742734 
L 414.49831 96.214087 
L 424.694746 96.266107 
L 426.734034 97.264715 
L 447.126907 97.430509 
L 455.284057 97.504723 
L 457.323344 104.22282 
L 459.362631 104.244912 
L 461.401919 104.938309 
L 463.441206 105.18449 
L 467.519781 105.416738 
L 469.559068 105.542748 
L 477.716217 105.654961 
L 479.755505 105.722351 
L 481.794792 105.971703 
L 483.834079 105.977907 
L 491.991229 106.56293 
L 498.109091 106.595183 
L 498.109091 106.595183 
" style="fill:none;stroke:#ff0000;stroke-dasharray:3,4.95;stroke-dashoffset:0;stroke-width:3;"/>
   </g>
   <g id="line2d_21">
    <path clip-path="url(#p163a1be3ee)" d="M 92.290909 67.236983 
L 96.369484 68.144301 
L 98.408771 68.46784 
L 100.448058 68.954091 
L 102.487346 69.278286 
L 104.526633 69.73314 
L 106.565921 70.320888 
L 108.605208 70.424299 
L 110.644495 70.808111 
L 112.683783 71.057335 
L 114.72307 71.680872 
L 116.762357 71.794354 
L 120.840932 72.685652 
L 124.919507 73.777707 
L 126.958794 73.964992 
L 128.998081 73.964992 
L 131.037369 74.753272 
L 133.076656 75.204012 
L 135.115943 75.777141 
L 137.155231 76.202951 
L 139.194518 76.229056 
L 145.31238 76.884576 
L 149.390955 77.991347 
L 151.430242 78.121126 
L 153.469529 78.585535 
L 155.508817 79.200639 
L 163.665966 80.127742 
L 165.705254 80.369802 
L 167.744541 80.40564 
L 169.783828 80.822015 
L 171.823116 81.022797 
L 173.862403 81.460564 
L 175.90169 81.668957 
L 177.940978 82.111932 
L 184.05884 82.291325 
L 186.098127 82.692116 
L 190.176702 83.268153 
L 196.294564 83.431011 
L 198.333851 83.65655 
L 204.451713 84.00615 
L 208.530288 84.163045 
L 210.569575 84.184668 
L 212.608862 84.703749 
L 214.64815 85.026166 
L 218.726725 85.286957 
L 220.766012 85.305081 
L 222.805299 85.51795 
L 239.119598 85.949248 
L 241.158885 86.165484 
L 261.551759 86.796655 
L 269.708908 86.869383 
L 271.748196 90.584961 
L 273.787483 90.618145 
L 275.82677 92.150555 
L 277.866058 92.949294 
L 286.023207 93.451026 
L 288.062494 94.489169 
L 290.101782 94.925605 
L 292.141069 95.245493 
L 296.219644 95.374173 
L 298.258931 96.225564 
L 300.298218 96.378112 
L 302.337506 96.780149 
L 304.376793 96.97705 
L 310.494655 98.273542 
L 312.533942 99.665461 
L 314.57323 99.665461 
L 320.691092 100.663065 
L 324.769667 101.466307 
L 326.808954 101.705123 
L 328.848241 102.787806 
L 330.887529 103.161792 
L 332.926816 103.178286 
L 337.005391 103.586695 
L 339.044678 104.115628 
L 341.083965 104.37362 
L 343.123253 105.106331 
L 345.16254 105.534732 
L 347.201827 106.252695 
L 351.280402 106.775609 
L 353.319689 106.775609 
L 361.476839 107.831337 
L 363.516126 107.935265 
L 365.555413 108.397527 
L 369.633988 108.910601 
L 373.712563 110.068573 
L 381.869712 110.826662 
L 383.909 111.166546 
L 385.948287 111.356516 
L 387.987574 111.965027 
L 390.026862 112.221071 
L 392.066149 112.593153 
L 396.144724 112.977956 
L 402.262586 113.260417 
L 406.34116 113.559033 
L 414.49831 113.865724 
L 416.537597 114.286518 
L 424.694746 114.598803 
L 426.734034 114.644831 
L 428.773321 115.691492 
L 434.891183 115.788319 
L 443.048333 115.923899 
L 445.08762 116.333585 
L 447.126907 117.921283 
L 449.166195 118.225086 
L 451.205482 118.862653 
L 453.244769 118.902552 
L 455.284057 119.443164 
L 461.401919 119.581903 
L 463.441206 119.690885 
L 465.480493 119.982612 
L 467.519781 120.568293 
L 469.559068 120.740896 
L 473.637643 120.795694 
L 475.67693 121.424091 
L 477.716217 121.636586 
L 483.834079 121.851299 
L 485.873367 121.864657 
L 487.912654 122.761613 
L 489.951942 122.942525 
L 496.069804 123.758061 
L 498.109091 123.872047 
L 498.109091 123.872047 
" style="fill:none;stroke:#1f77b4;stroke-dasharray:19.2,4.8,3,4.8;stroke-dashoffset:0;stroke-width:3;"/>
    <defs>
     <path d="M 0 -3 
L -2.85317 -0.927051 
L -1.763356 2.427051 
L 1.763356 2.427051 
L 2.85317 -0.927051 
z
" id="mf69f4d7cf9" style="stroke:#1f77b4;stroke-linejoin:miter;"/>
    </defs>
    <g clip-path="url(#p163a1be3ee)">
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="92.290909" xlink:href="#mf69f4d7cf9" y="67.236983"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="94.330196" xlink:href="#mf69f4d7cf9" y="67.703283"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="96.369484" xlink:href="#mf69f4d7cf9" y="68.144301"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="98.408771" xlink:href="#mf69f4d7cf9" y="68.46784"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="100.448058" xlink:href="#mf69f4d7cf9" y="68.954091"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="102.487346" xlink:href="#mf69f4d7cf9" y="69.278286"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="104.526633" xlink:href="#mf69f4d7cf9" y="69.73314"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="106.565921" xlink:href="#mf69f4d7cf9" y="70.320888"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="108.605208" xlink:href="#mf69f4d7cf9" y="70.424299"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="110.644495" xlink:href="#mf69f4d7cf9" y="70.808111"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="112.683783" xlink:href="#mf69f4d7cf9" y="71.057335"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="114.72307" xlink:href="#mf69f4d7cf9" y="71.680872"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="116.762357" xlink:href="#mf69f4d7cf9" y="71.794354"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="118.801645" xlink:href="#mf69f4d7cf9" y="72.228437"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="120.840932" xlink:href="#mf69f4d7cf9" y="72.685652"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="122.880219" xlink:href="#mf69f4d7cf9" y="73.250971"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="124.919507" xlink:href="#mf69f4d7cf9" y="73.777707"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="126.958794" xlink:href="#mf69f4d7cf9" y="73.964992"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="128.998081" xlink:href="#mf69f4d7cf9" y="73.964992"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="131.037369" xlink:href="#mf69f4d7cf9" y="74.753272"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="133.076656" xlink:href="#mf69f4d7cf9" y="75.204012"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="135.115943" xlink:href="#mf69f4d7cf9" y="75.777141"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="137.155231" xlink:href="#mf69f4d7cf9" y="76.202951"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="139.194518" xlink:href="#mf69f4d7cf9" y="76.229056"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="141.233805" xlink:href="#mf69f4d7cf9" y="76.452171"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="143.273093" xlink:href="#mf69f4d7cf9" y="76.59064"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="145.31238" xlink:href="#mf69f4d7cf9" y="76.884576"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="147.351667" xlink:href="#mf69f4d7cf9" y="77.441301"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="149.390955" xlink:href="#mf69f4d7cf9" y="77.991347"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="151.430242" xlink:href="#mf69f4d7cf9" y="78.121126"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="153.469529" xlink:href="#mf69f4d7cf9" y="78.585535"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="155.508817" xlink:href="#mf69f4d7cf9" y="79.200639"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="157.548104" xlink:href="#mf69f4d7cf9" y="79.406365"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="159.587392" xlink:href="#mf69f4d7cf9" y="79.62335"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="161.626679" xlink:href="#mf69f4d7cf9" y="79.876942"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="163.665966" xlink:href="#mf69f4d7cf9" y="80.127742"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="165.705254" xlink:href="#mf69f4d7cf9" y="80.369802"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="167.744541" xlink:href="#mf69f4d7cf9" y="80.40564"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="169.783828" xlink:href="#mf69f4d7cf9" y="80.822015"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="171.823116" xlink:href="#mf69f4d7cf9" y="81.022797"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="173.862403" xlink:href="#mf69f4d7cf9" y="81.460564"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="175.90169" xlink:href="#mf69f4d7cf9" y="81.668957"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="177.940978" xlink:href="#mf69f4d7cf9" y="82.111932"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="179.980265" xlink:href="#mf69f4d7cf9" y="82.208736"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="182.019552" xlink:href="#mf69f4d7cf9" y="82.229571"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="184.05884" xlink:href="#mf69f4d7cf9" y="82.291325"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="186.098127" xlink:href="#mf69f4d7cf9" y="82.692116"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="188.137414" xlink:href="#mf69f4d7cf9" y="82.929778"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="190.176702" xlink:href="#mf69f4d7cf9" y="83.268153"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="192.215989" xlink:href="#mf69f4d7cf9" y="83.291474"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="194.255276" xlink:href="#mf69f4d7cf9" y="83.375476"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="196.294564" xlink:href="#mf69f4d7cf9" y="83.431011"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="198.333851" xlink:href="#mf69f4d7cf9" y="83.65655"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="200.373138" xlink:href="#mf69f4d7cf9" y="83.739935"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="202.412426" xlink:href="#mf69f4d7cf9" y="83.88307"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="204.451713" xlink:href="#mf69f4d7cf9" y="84.00615"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="206.491" xlink:href="#mf69f4d7cf9" y="84.139453"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="208.530288" xlink:href="#mf69f4d7cf9" y="84.163045"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="210.569575" xlink:href="#mf69f4d7cf9" y="84.184668"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="212.608862" xlink:href="#mf69f4d7cf9" y="84.703749"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="214.64815" xlink:href="#mf69f4d7cf9" y="85.026166"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="216.687437" xlink:href="#mf69f4d7cf9" y="85.187578"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="218.726725" xlink:href="#mf69f4d7cf9" y="85.286957"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="220.766012" xlink:href="#mf69f4d7cf9" y="85.305081"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="222.805299" xlink:href="#mf69f4d7cf9" y="85.51795"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="224.844587" xlink:href="#mf69f4d7cf9" y="85.565286"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="226.883874" xlink:href="#mf69f4d7cf9" y="85.652497"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="228.923161" xlink:href="#mf69f4d7cf9" y="85.692993"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="230.962449" xlink:href="#mf69f4d7cf9" y="85.716541"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="233.001736" xlink:href="#mf69f4d7cf9" y="85.766759"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="235.041023" xlink:href="#mf69f4d7cf9" y="85.895224"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="237.080311" xlink:href="#mf69f4d7cf9" y="85.916111"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="239.119598" xlink:href="#mf69f4d7cf9" y="85.949248"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="241.158885" xlink:href="#mf69f4d7cf9" y="86.165484"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="243.198173" xlink:href="#mf69f4d7cf9" y="86.239473"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="245.23746" xlink:href="#mf69f4d7cf9" y="86.29844"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="247.276747" xlink:href="#mf69f4d7cf9" y="86.325058"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="249.316035" xlink:href="#mf69f4d7cf9" y="86.445902"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="251.355322" xlink:href="#mf69f4d7cf9" y="86.494899"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="253.394609" xlink:href="#mf69f4d7cf9" y="86.557775"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="255.433897" xlink:href="#mf69f4d7cf9" y="86.716485"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="257.473184" xlink:href="#mf69f4d7cf9" y="86.738574"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="259.512471" xlink:href="#mf69f4d7cf9" y="86.748596"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="261.551759" xlink:href="#mf69f4d7cf9" y="86.796655"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="263.591046" xlink:href="#mf69f4d7cf9" y="86.81517"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="265.630333" xlink:href="#mf69f4d7cf9" y="86.857444"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="267.669621" xlink:href="#mf69f4d7cf9" y="86.865281"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="269.708908" xlink:href="#mf69f4d7cf9" y="86.869383"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="271.748196" xlink:href="#mf69f4d7cf9" y="90.584961"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="273.787483" xlink:href="#mf69f4d7cf9" y="90.618145"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="275.82677" xlink:href="#mf69f4d7cf9" y="92.150555"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="277.866058" xlink:href="#mf69f4d7cf9" y="92.949294"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="279.905345" xlink:href="#mf69f4d7cf9" y="93.102542"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="281.944632" xlink:href="#mf69f4d7cf9" y="93.285274"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="283.98392" xlink:href="#mf69f4d7cf9" y="93.381505"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="286.023207" xlink:href="#mf69f4d7cf9" y="93.451026"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="288.062494" xlink:href="#mf69f4d7cf9" y="94.489169"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="290.101782" xlink:href="#mf69f4d7cf9" y="94.925605"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="292.141069" xlink:href="#mf69f4d7cf9" y="95.245493"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="294.180356" xlink:href="#mf69f4d7cf9" y="95.274212"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="296.219644" xlink:href="#mf69f4d7cf9" y="95.374173"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="298.258931" xlink:href="#mf69f4d7cf9" y="96.225564"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="300.298218" xlink:href="#mf69f4d7cf9" y="96.378112"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="302.337506" xlink:href="#mf69f4d7cf9" y="96.780149"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="304.376793" xlink:href="#mf69f4d7cf9" y="96.97705"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="306.41608" xlink:href="#mf69f4d7cf9" y="97.437359"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="308.455368" xlink:href="#mf69f4d7cf9" y="97.960492"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="310.494655" xlink:href="#mf69f4d7cf9" y="98.273542"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="312.533942" xlink:href="#mf69f4d7cf9" y="99.665461"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="314.57323" xlink:href="#mf69f4d7cf9" y="99.665461"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="316.612517" xlink:href="#mf69f4d7cf9" y="99.972127"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="318.651804" xlink:href="#mf69f4d7cf9" y="100.345524"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="320.691092" xlink:href="#mf69f4d7cf9" y="100.663065"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="322.730379" xlink:href="#mf69f4d7cf9" y="101.084037"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="324.769667" xlink:href="#mf69f4d7cf9" y="101.466307"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="326.808954" xlink:href="#mf69f4d7cf9" y="101.705123"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="328.848241" xlink:href="#mf69f4d7cf9" y="102.787806"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="330.887529" xlink:href="#mf69f4d7cf9" y="103.161792"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="332.926816" xlink:href="#mf69f4d7cf9" y="103.178286"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="334.966103" xlink:href="#mf69f4d7cf9" y="103.437385"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="337.005391" xlink:href="#mf69f4d7cf9" y="103.586695"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="339.044678" xlink:href="#mf69f4d7cf9" y="104.115628"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="341.083965" xlink:href="#mf69f4d7cf9" y="104.37362"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="343.123253" xlink:href="#mf69f4d7cf9" y="105.106331"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="345.16254" xlink:href="#mf69f4d7cf9" y="105.534732"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="347.201827" xlink:href="#mf69f4d7cf9" y="106.252695"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="349.241115" xlink:href="#mf69f4d7cf9" y="106.529084"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="351.280402" xlink:href="#mf69f4d7cf9" y="106.775609"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="353.319689" xlink:href="#mf69f4d7cf9" y="106.775609"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="355.358977" xlink:href="#mf69f4d7cf9" y="107.034869"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="357.398264" xlink:href="#mf69f4d7cf9" y="107.299791"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="359.437551" xlink:href="#mf69f4d7cf9" y="107.596197"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="361.476839" xlink:href="#mf69f4d7cf9" y="107.831337"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="363.516126" xlink:href="#mf69f4d7cf9" y="107.935265"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="365.555413" xlink:href="#mf69f4d7cf9" y="108.397527"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="367.594701" xlink:href="#mf69f4d7cf9" y="108.633923"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="369.633988" xlink:href="#mf69f4d7cf9" y="108.910601"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="371.673275" xlink:href="#mf69f4d7cf9" y="109.455066"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="373.712563" xlink:href="#mf69f4d7cf9" y="110.068573"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="375.75185" xlink:href="#mf69f4d7cf9" y="110.248633"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="377.791138" xlink:href="#mf69f4d7cf9" y="110.378743"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="379.830425" xlink:href="#mf69f4d7cf9" y="110.60821"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="381.869712" xlink:href="#mf69f4d7cf9" y="110.826662"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="383.909" xlink:href="#mf69f4d7cf9" y="111.166546"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="385.948287" xlink:href="#mf69f4d7cf9" y="111.356516"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="387.987574" xlink:href="#mf69f4d7cf9" y="111.965027"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="390.026862" xlink:href="#mf69f4d7cf9" y="112.221071"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="392.066149" xlink:href="#mf69f4d7cf9" y="112.593153"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="394.105436" xlink:href="#mf69f4d7cf9" y="112.786481"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="396.144724" xlink:href="#mf69f4d7cf9" y="112.977956"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="398.184011" xlink:href="#mf69f4d7cf9" y="113.040976"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="400.223298" xlink:href="#mf69f4d7cf9" y="113.167274"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="402.262586" xlink:href="#mf69f4d7cf9" y="113.260417"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="404.301873" xlink:href="#mf69f4d7cf9" y="113.448413"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="406.34116" xlink:href="#mf69f4d7cf9" y="113.559033"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="408.380448" xlink:href="#mf69f4d7cf9" y="113.640655"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="410.419735" xlink:href="#mf69f4d7cf9" y="113.761213"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="412.459022" xlink:href="#mf69f4d7cf9" y="113.804853"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="414.49831" xlink:href="#mf69f4d7cf9" y="113.865724"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="416.537597" xlink:href="#mf69f4d7cf9" y="114.286518"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="418.576884" xlink:href="#mf69f4d7cf9" y="114.382057"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="420.616172" xlink:href="#mf69f4d7cf9" y="114.412984"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="422.655459" xlink:href="#mf69f4d7cf9" y="114.537211"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="424.694746" xlink:href="#mf69f4d7cf9" y="114.598803"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="426.734034" xlink:href="#mf69f4d7cf9" y="114.644831"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="428.773321" xlink:href="#mf69f4d7cf9" y="115.691492"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="430.812608" xlink:href="#mf69f4d7cf9" y="115.749954"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="432.851896" xlink:href="#mf69f4d7cf9" y="115.786199"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="434.891183" xlink:href="#mf69f4d7cf9" y="115.788319"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="436.930471" xlink:href="#mf69f4d7cf9" y="115.7945"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="438.969758" xlink:href="#mf69f4d7cf9" y="115.900397"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="441.009045" xlink:href="#mf69f4d7cf9" y="115.914304"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="443.048333" xlink:href="#mf69f4d7cf9" y="115.923899"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="445.08762" xlink:href="#mf69f4d7cf9" y="116.333585"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="447.126907" xlink:href="#mf69f4d7cf9" y="117.921283"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="449.166195" xlink:href="#mf69f4d7cf9" y="118.225086"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="451.205482" xlink:href="#mf69f4d7cf9" y="118.862653"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="453.244769" xlink:href="#mf69f4d7cf9" y="118.902552"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="455.284057" xlink:href="#mf69f4d7cf9" y="119.443164"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="457.323344" xlink:href="#mf69f4d7cf9" y="119.471565"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="459.362631" xlink:href="#mf69f4d7cf9" y="119.512104"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="461.401919" xlink:href="#mf69f4d7cf9" y="119.581903"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="463.441206" xlink:href="#mf69f4d7cf9" y="119.690885"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="465.480493" xlink:href="#mf69f4d7cf9" y="119.982612"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="467.519781" xlink:href="#mf69f4d7cf9" y="120.568293"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="469.559068" xlink:href="#mf69f4d7cf9" y="120.740896"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="471.598355" xlink:href="#mf69f4d7cf9" y="120.761744"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="473.637643" xlink:href="#mf69f4d7cf9" y="120.795694"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="475.67693" xlink:href="#mf69f4d7cf9" y="121.424091"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="477.716217" xlink:href="#mf69f4d7cf9" y="121.636586"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="479.755505" xlink:href="#mf69f4d7cf9" y="121.736082"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="481.794792" xlink:href="#mf69f4d7cf9" y="121.851299"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="483.834079" xlink:href="#mf69f4d7cf9" y="121.851299"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="485.873367" xlink:href="#mf69f4d7cf9" y="121.864657"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="487.912654" xlink:href="#mf69f4d7cf9" y="122.761613"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="489.951942" xlink:href="#mf69f4d7cf9" y="122.942525"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="491.991229" xlink:href="#mf69f4d7cf9" y="123.250014"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="494.030516" xlink:href="#mf69f4d7cf9" y="123.644951"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="496.069804" xlink:href="#mf69f4d7cf9" y="123.758061"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="498.109091" xlink:href="#mf69f4d7cf9" y="123.872047"/>
    </g>
   </g>
   <g id="patch_3">
    <path d="M 72 378 
L 72 51.84 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="patch_4">
    <path d="M 518.4 378 
L 518.4 51.84 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="patch_5">
    <path d="M 72 378 
L 518.4 378 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="patch_6">
    <path d="M 72 51.84 
L 518.4 51.84 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="legend_1">
    <g id="patch_7">
     <path d="M 82.5 370.5 
L 176.446875 370.5 
Q 179.446875 370.5 179.446875 367.5 
L 179.446875 280.93125 
Q 179.446875 277.93125 176.446875 277.93125 
L 82.5 277.93125 
Q 79.5 277.93125 79.5 280.93125 
L 79.5 367.5 
Q 79.5 370.5 82.5 370.5 
z
" style="fill:#ffffff;opacity:0.8;stroke:#cccccc;stroke-linejoin:miter;"/>
    </g>
    <g id="line2d_22">
     <path d="M 85.5 290.078906 
L 115.5 290.078906 
" style="fill:none;stroke:#0000ff;stroke-linecap:square;stroke-width:3;"/>
    </g>
    <g id="line2d_23"/>
    <g id="text_20">
     <!-- p=0.2 -->
     <g transform="translate(127.5 295.328906)scale(0.15 -0.15)">
      <defs>
       <path d="M 1159 525 
L 1159 -1331 
L 581 -1331 
L 581 3500 
L 1159 3500 
L 1159 2969 
Q 1341 3281 1617 3432 
Q 1894 3584 2278 3584 
Q 2916 3584 3314 3078 
Q 3713 2572 3713 1747 
Q 3713 922 3314 415 
Q 2916 -91 2278 -91 
Q 1894 -91 1617 61 
Q 1341 213 1159 525 
z
M 3116 1747 
Q 3116 2381 2855 2742 
Q 2594 3103 2138 3103 
Q 1681 3103 1420 2742 
Q 1159 2381 1159 1747 
Q 1159 1113 1420 752 
Q 1681 391 2138 391 
Q 2594 391 2855 752 
Q 3116 1113 3116 1747 
z
" id="DejaVuSans-70" transform="scale(0.015625)"/>
       <path d="M 678 2906 
L 4684 2906 
L 4684 2381 
L 678 2381 
L 678 2906 
z
M 678 1631 
L 4684 1631 
L 4684 1100 
L 678 1100 
L 678 1631 
z
" id="DejaVuSans-3d" transform="scale(0.015625)"/>
       <path d="M 684 794 
L 1344 794 
L 1344 0 
L 684 0 
L 684 794 
z
" id="DejaVuSans-2e" transform="scale(0.015625)"/>
      </defs>
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-30"/>
      <use x="210.888672" xlink:href="#DejaVuSans-2e"/>
      <use x="242.675781" xlink:href="#DejaVuSans-32"/>
     </g>
    </g>
    <g id="line2d_24">
     <path d="M 85.5 312.096094 
L 115.5 312.096094 
" style="fill:none;stroke:#008000;stroke-dasharray:11.1,4.8;stroke-dashoffset:0;stroke-width:3;"/>
    </g>
    <g id="line2d_25"/>
    <g id="text_21">
     <!-- p=0.4 -->
     <g transform="translate(127.5 317.346094)scale(0.15 -0.15)">
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-30"/>
      <use x="210.888672" xlink:href="#DejaVuSans-2e"/>
      <use x="242.675781" xlink:href="#DejaVuSans-34"/>
     </g>
    </g>
    <g id="line2d_26">
     <path d="M 85.5 334.113281 
L 115.5 334.113281 
" style="fill:none;stroke:#ff0000;stroke-dasharray:3,4.95;stroke-dashoffset:0;stroke-width:3;"/>
    </g>
    <g id="line2d_27"/>
    <g id="text_22">
     <!-- p=0.6 -->
     <g transform="translate(127.5 339.363281)scale(0.15 -0.15)">
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-30"/>
      <use x="210.888672" xlink:href="#DejaVuSans-2e"/>
      <use x="242.675781" xlink:href="#DejaVuSans-36"/>
     </g>
    </g>
    <g id="line2d_28">
     <path d="M 85.5 356.130469 
L 115.5 356.130469 
" style="fill:none;stroke:#1f77b4;stroke-dasharray:19.2,4.8,3,4.8;stroke-dashoffset:0;stroke-width:3;"/>
    </g>
    <g id="line2d_29">
     <g>
      <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="100.5" xlink:href="#mf69f4d7cf9" y="356.130469"/>
     </g>
    </g>
    <g id="text_23">
     <!-- p=1 -->
     <g transform="translate(127.5 361.380469)scale(0.15 -0.15)">
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-31"/>
     </g>
    </g>
   </g>
  </g>
 </g>
 <defs>
  <clipPath id="p163a1be3ee">
   <rect height="326.16" width="446.4" x="72" y="51.84"/>
  </clipPath>
 </defs>
</svg>


==> figs/p04_all_methods <==
<?xml version="1.0" encoding="utf-8" standalone="no"?>
<!DOCTYPE svg PUBLIC "-//W3C//DTD SVG 1.1//EN"
  "http://www.w3.org/Graphics/SVG/1.1/DTD/svg11.dtd">
<svg height="432pt" version="1.1" viewBox="0 0 576 432" width="576pt" xmlns="http://www.w3.org/2000/svg" xmlns:xlink="http://www.w3.org/1999/xlink">
 <metadata>
  <rdf:RDF xmlns:cc="http://creativecommons.org/ns#" xmlns:dc="http://purl.org/dc/elements/1.1/" xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#">
   <cc:Work>
    <dc:type rdf:resource="http://purl.org/dc/dcmitype/StillImage"/>
    <dc:date>2021-10-19T15:48:20.442835</dc:date>
    <dc:format>image/svg+xml</dc:format>
    <dc:creator>
     <cc:Agent>
      <dc:title>Matplotlib v3.4.2, https://matplotlib.org/</dc:title>
     </cc:Agent>
    </dc:creator>
   </cc:Work>
  </rdf:RDF>
 </metadata>
 <defs>
  <style type="text/css">*{stroke-linecap:butt;stroke-linejoin:round;}</style>
 </defs>
 <g id="figure_1">
  <g id="patch_1">
   <path d="M 0 432 
L 576 432 
L 576 0 
L 0 0 
z
" style="fill:none;"/>
  </g>
  <g id="axes_1">
   <g id="patch_2">
    <path d="M 72 378 
L 518.4 378 
L 518.4 51.84 
L 72 51.84 
z
" style="fill:#ffffff;"/>
   </g>
   <g id="matplotlib.axis_1">
    <g id="xtick_1">
     <g id="line2d_1">
      <defs>
       <path d="M 0 0 
L 0 3.5 
" id="m32c7ddd424" style="stroke:#000000;stroke-width:0.8;"/>
      </defs>
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="92.290909" xlink:href="#m32c7ddd424" y="378"/>
      </g>
     </g>
     <g id="text_1">
      <!-- 0 -->
      <g transform="translate(87.519034 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 2034 4250 
Q 1547 4250 1301 3770 
Q 1056 3291 1056 2328 
Q 1056 1369 1301 889 
Q 1547 409 2034 409 
Q 2525 409 2770 889 
Q 3016 1369 3016 2328 
Q 3016 3291 2770 3770 
Q 2525 4250 2034 4250 
z
M 2034 4750 
Q 2819 4750 3233 4129 
Q 3647 3509 3647 2328 
Q 3647 1150 3233 529 
Q 2819 -91 2034 -91 
Q 1250 -91 836 529 
Q 422 1150 422 2328 
Q 422 3509 836 4129 
Q 1250 4750 2034 4750 
z
" id="DejaVuSans-30" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_2">
     <g id="line2d_2">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="143.273093" xlink:href="#m32c7ddd424" y="378"/>
      </g>
     </g>
     <g id="text_2">
      <!-- 25 -->
      <g transform="translate(133.729343 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 1228 531 
L 3431 531 
L 3431 0 
L 469 0 
L 469 531 
Q 828 903 1448 1529 
Q 2069 2156 2228 2338 
Q 2531 2678 2651 2914 
Q 2772 3150 2772 3378 
Q 2772 3750 2511 3984 
Q 2250 4219 1831 4219 
Q 1534 4219 1204 4116 
Q 875 4013 500 3803 
L 500 4441 
Q 881 4594 1212 4672 
Q 1544 4750 1819 4750 
Q 2544 4750 2975 4387 
Q 3406 4025 3406 3419 
Q 3406 3131 3298 2873 
Q 3191 2616 2906 2266 
Q 2828 2175 2409 1742 
Q 1991 1309 1228 531 
z
" id="DejaVuSans-32" transform="scale(0.015625)"/>
        <path d="M 691 4666 
L 3169 4666 
L 3169 4134 
L 1269 4134 
L 1269 2991 
Q 1406 3038 1543 3061 
Q 1681 3084 1819 3084 
Q 2600 3084 3056 2656 
Q 3513 2228 3513 1497 
Q 3513 744 3044 326 
Q 2575 -91 1722 -91 
Q 1428 -91 1123 -41 
Q 819 9 494 109 
L 494 744 
Q 775 591 1075 516 
Q 1375 441 1709 441 
Q 2250 441 2565 725 
Q 2881 1009 2881 1497 
Q 2881 1984 2565 2268 
Q 2250 2553 1709 2553 
Q 1456 2553 1204 2497 
Q 953 2441 691 2322 
L 691 4666 
z
" id="DejaVuSans-35" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-32"/>
       <use x="63.623047" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_3">
     <g id="line2d_3">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="194.255276" xlink:href="#m32c7ddd424" y="378"/>
      </g>
     </g>
     <g id="text_3">
      <!-- 50 -->
      <g transform="translate(184.711526 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-35"/>
       <use x="63.623047" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_4">
     <g id="line2d_4">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="245.23746" xlink:href="#m32c7ddd424" y="378"/>
      </g>
     </g>
     <g id="text_4">
      <!-- 75 -->
      <g transform="translate(235.69371 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 525 4666 
L 3525 4666 
L 3525 4397 
L 1831 0 
L 1172 0 
L 2766 4134 
L 525 4134 
L 525 4666 
z
" id="DejaVuSans-37" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-37"/>
       <use x="63.623047" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_5">
     <g id="line2d_5">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="296.219644" xlink:href="#m32c7ddd424" y="378"/>
      </g>
     </g>
     <g id="text_5">
      <!-- 100 -->
      <g transform="translate(281.904019 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 794 531 
L 1825 531 
L 1825 4091 
L 703 3866 
L 703 4441 
L 1819 4666 
L 2450 4666 
L 2450 531 
L 3481 531 
L 3481 0 
L 794 0 
L 794 531 
z
" id="DejaVuSans-31" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-30"/>
       <use x="127.246094" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_6">
     <g id="line2d_6">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="347.201827" xlink:href="#m32c7ddd424" y="378"/>
      </g>
     </g>
     <g id="text_6">
      <!-- 125 -->
      <g transform="translate(332.886202 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-32"/>
       <use x="127.246094" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_7">
     <g id="line2d_7">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="398.184011" xlink:href="#m32c7ddd424" y="378"/>
      </g>
     </g>
     <g id="text_7">
      <!-- 150 -->
      <g transform="translate(383.868386 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-35"/>
       <use x="127.246094" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_8">
     <g id="line2d_8">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="449.166195" xlink:href="#m32c7ddd424" y="378"/>
      </g>
     </g>
     <g id="text_8">
      <!-- 175 -->
      <g transform="translate(434.85057 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-37"/>
       <use x="127.246094" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_9">
     <g id="line2d_9">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="500.148378" xlink:href="#m32c7ddd424" y="378"/>
      </g>
     </g>
     <g id="text_9">
      <!-- 200 -->
      <g transform="translate(485.832753 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-32"/>
       <use x="63.623047" xlink:href="#DejaVuSans-30"/>
       <use x="127.246094" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="text_10">
     <!-- Iteration number, $k$ -->
     <g transform="translate(222.6 414.914844)scale(0.15 -0.15)">
      <defs>
       <path d="M 628 4666 
L 1259 4666 
L 1259 0 
L 628 0 
L 628 4666 
z
" id="DejaVuSans-49" transform="scale(0.015625)"/>
       <path d="M 1172 4494 
L 1172 3500 
L 2356 3500 
L 2356 3053 
L 1172 3053 
L 1172 1153 
Q 1172 725 1289 603 
Q 1406 481 1766 481 
L 2356 481 
L 2356 0 
L 1766 0 
Q 1100 0 847 248 
Q 594 497 594 1153 
L 594 3053 
L 172 3053 
L 172 3500 
L 594 3500 
L 594 4494 
L 1172 4494 
z
" id="DejaVuSans-74" transform="scale(0.015625)"/>
       <path d="M 3597 1894 
L 3597 1613 
L 953 1613 
Q 991 1019 1311 708 
Q 1631 397 2203 397 
Q 2534 397 2845 478 
Q 3156 559 3463 722 
L 3463 178 
Q 3153 47 2828 -22 
Q 2503 -91 2169 -91 
Q 1331 -91 842 396 
Q 353 884 353 1716 
Q 353 2575 817 3079 
Q 1281 3584 2069 3584 
Q 2775 3584 3186 3129 
Q 3597 2675 3597 1894 
z
M 3022 2063 
Q 3016 2534 2758 2815 
Q 2500 3097 2075 3097 
Q 1594 3097 1305 2825 
Q 1016 2553 972 2059 
L 3022 2063 
z
" id="DejaVuSans-65" transform="scale(0.015625)"/>
       <path d="M 2631 2963 
Q 2534 3019 2420 3045 
Q 2306 3072 2169 3072 
Q 1681 3072 1420 2755 
Q 1159 2438 1159 1844 
L 1159 0 
L 581 0 
L 581 3500 
L 1159 3500 
L 1159 2956 
Q 1341 3275 1631 3429 
Q 1922 3584 2338 3584 
Q 2397 3584 2469 3576 
Q 2541 3569 2628 3553 
L 2631 2963 
z
" id="DejaVuSans-72" transform="scale(0.015625)"/>
       <path d="M 2194 1759 
Q 1497 1759 1228 1600 
Q 959 1441 959 1056 
Q 959 750 1161 570 
Q 1363 391 1709 391 
Q 2188 391 2477 730 
Q 2766 1069 2766 1631 
L 2766 1759 
L 2194 1759 
z
M 3341 1997 
L 3341 0 
L 2766 0 
L 2766 531 
Q 2569 213 2275 61 
Q 1981 -91 1556 -91 
Q 1019 -91 701 211 
Q 384 513 384 1019 
Q 384 1609 779 1909 
Q 1175 2209 1959 2209 
L 2766 2209 
L 2766 2266 
Q 2766 2663 2505 2880 
Q 2244 3097 1772 3097 
Q 1472 3097 1187 3025 
Q 903 2953 641 2809 
L 641 3341 
Q 956 3463 1253 3523 
Q 1550 3584 1831 3584 
Q 2591 3584 2966 3190 
Q 3341 2797 3341 1997 
z
" id="DejaVuSans-61" transform="scale(0.015625)"/>
       <path d="M 603 3500 
L 1178 3500 
L 1178 0 
L 603 0 
L 603 3500 
z
M 603 4863 
L 1178 4863 
L 1178 4134 
L 603 4134 
L 603 4863 
z
" id="DejaVuSans-69" transform="scale(0.015625)"/>
       <path d="M 1959 3097 
Q 1497 3097 1228 2736 
Q 959 2375 959 1747 
Q 959 1119 1226 758 
Q 1494 397 1959 397 
Q 2419 397 2687 759 
Q 2956 1122 2956 1747 
Q 2956 2369 2687 2733 
Q 2419 3097 1959 3097 
z
M 1959 3584 
Q 2709 3584 3137 3096 
Q 3566 2609 3566 1747 
Q 3566 888 3137 398 
Q 2709 -91 1959 -91 
Q 1206 -91 779 398 
Q 353 888 353 1747 
Q 353 2609 779 3096 
Q 1206 3584 1959 3584 
z
" id="DejaVuSans-6f" transform="scale(0.015625)"/>
       <path d="M 3513 2113 
L 3513 0 
L 2938 0 
L 2938 2094 
Q 2938 2591 2744 2837 
Q 2550 3084 2163 3084 
Q 1697 3084 1428 2787 
Q 1159 2491 1159 1978 
L 1159 0 
L 581 0 
L 581 3500 
L 1159 3500 
L 1159 2956 
Q 1366 3272 1645 3428 
Q 1925 3584 2291 3584 
Q 2894 3584 3203 3211 
Q 3513 2838 3513 2113 
z
" id="DejaVuSans-6e" transform="scale(0.015625)"/>
       <path id="DejaVuSans-20" transform="scale(0.015625)"/>
       <path d="M 544 1381 
L 544 3500 
L 1119 3500 
L 1119 1403 
Q 1119 906 1312 657 
Q 1506 409 1894 409 
Q 2359 409 2629 706 
Q 2900 1003 2900 1516 
L 2900 3500 
L 3475 3500 
L 3475 0 
L 2900 0 
L 2900 538 
Q 2691 219 2414 64 
Q 2138 -91 1772 -91 
Q 1169 -91 856 284 
Q 544 659 544 1381 
z
M 1991 3584 
L 1991 3584 
z
" id="DejaVuSans-75" transform="scale(0.015625)"/>
       <path d="M 3328 2828 
Q 3544 3216 3844 3400 
Q 4144 3584 4550 3584 
Q 5097 3584 5394 3201 
Q 5691 2819 5691 2113 
L 5691 0 
L 5113 0 
L 5113 2094 
Q 5113 2597 4934 2840 
Q 4756 3084 4391 3084 
Q 3944 3084 3684 2787 
Q 3425 2491 3425 1978 
L 3425 0 
L 2847 0 
L 2847 2094 
Q 2847 2600 2669 2842 
Q 2491 3084 2119 3084 
Q 1678 3084 1418 2786 
Q 1159 2488 1159 1978 
L 1159 0 
L 581 0 
L 581 3500 
L 1159 3500 
L 1159 2956 
Q 1356 3278 1631 3431 
Q 1906 3584 2284 3584 
Q 2666 3584 2933 3390 
Q 3200 3197 3328 2828 
z
" id="DejaVuSans-6d" transform="scale(0.015625)"/>
       <path d="M 3116 1747 
Q 3116 2381 2855 2742 
Q 2594 3103 2138 3103 
Q 1681 3103 1420 2742 
Q 1159 2381 1159 1747 
Q 1159 1113 1420 752 
Q 1681 391 2138 391 
Q 2594 391 2855 752 
Q 3116 1113 3116 1747 
z
M 1159 2969 
Q 1341 3281 1617 3432 
Q 1894 3584 2278 3584 
Q 2916 3584 3314 3078 
Q 3713 2572 3713 1747 
Q 3713 922 3314 415 
Q 2916 -91 2278 -91 
Q 1894 -91 1617 61 
Q 1341 213 1159 525 
L 1159 0 
L 581 0 
L 581 4863 
L 1159 4863 
L 1159 2969 
z
" id="DejaVuSans-62" transform="scale(0.015625)"/>
       <path d="M 750 794 
L 1409 794 
L 1409 256 
L 897 -744 
L 494 -744 
L 750 256 
L 750 794 
z
" id="DejaVuSans-2c" transform="scale(0.015625)"/>
       <path d="M 1172 4863 
L 1747 4863 
L 1197 2028 
L 3169 3500 
L 3916 3500 
L 1716 1825 
L 3322 0 
L 2625 0 
L 1131 1709 
L 800 0 
L 225 0 
L 1172 4863 
z
" id="DejaVuSans-Oblique-6b" transform="scale(0.015625)"/>
      </defs>
      <use transform="translate(0 0.015625)" xlink:href="#DejaVuSans-49"/>
      <use transform="translate(29.492188 0.015625)" xlink:href="#DejaVuSans-74"/>
      <use transform="translate(68.701172 0.015625)" xlink:href="#DejaVuSans-65"/>
      <use transform="translate(130.224609 0.015625)" xlink:href="#DejaVuSans-72"/>
      <use transform="translate(171.337891 0.015625)" xlink:href="#DejaVuSans-61"/>
      <use transform="translate(232.617188 0.015625)" xlink:href="#DejaVuSans-74"/>
      <use transform="translate(271.826172 0.015625)" xlink:href="#DejaVuSans-69"/>
      <use transform="translate(299.609375 0.015625)" xlink:href="#DejaVuSans-6f"/>
      <use transform="translate(360.791016 0.015625)" xlink:href="#DejaVuSans-6e"/>
      <use transform="translate(424.169922 0.015625)" xlink:href="#DejaVuSans-20"/>
      <use transform="translate(455.957031 0.015625)" xlink:href="#DejaVuSans-6e"/>
      <use transform="translate(519.335938 0.015625)" xlink:href="#DejaVuSans-75"/>
      <use transform="translate(582.714844 0.015625)" xlink:href="#DejaVuSans-6d"/>
      <use transform="translate(680.126953 0.015625)" xlink:href="#DejaVuSans-62"/>
      <use transform="translate(743.603516 0.015625)" xlink:href="#DejaVuSans-65"/>
      <use transform="translate(805.126953 0.015625)" xlink:href="#DejaVuSans-72"/>
      <use transform="translate(846.240234 0.015625)" xlink:href="#DejaVuSans-2c"/>
      <use transform="translate(878.027344 0.015625)" xlink:href="#DejaVuSans-20"/>
      <use transform="translate(909.814453 0.015625)" xlink:href="#DejaVuSans-Oblique-6b"/>
     </g>
    </g>
   </g>
   <g id="matplotlib.axis_2">
    <g id="ytick_1">
     <g id="line2d_10">
      <defs>
       <path d="M 0 0 
L -3.5 0 
" id="m09ba2c1beb" style="stroke:#000000;stroke-width:0.8;"/>
      </defs>
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m09ba2c1beb" y="341.095191"/>
      </g>
     </g>
     <g id="text_11">
      <!-- $\mathdefault{10^{-30}}$ -->
      <g transform="translate(23.15 346.794019)scale(0.15 -0.15)">
       <defs>
        <path d="M 678 2272 
L 4684 2272 
L 4684 1741 
L 678 1741 
L 678 2272 
z
" id="DejaVuSans-2212" transform="scale(0.015625)"/>
        <path d="M 2597 2516 
Q 3050 2419 3304 2112 
Q 3559 1806 3559 1356 
Q 3559 666 3084 287 
Q 2609 -91 1734 -91 
Q 1441 -91 1130 -33 
Q 819 25 488 141 
L 488 750 
Q 750 597 1062 519 
Q 1375 441 1716 441 
Q 2309 441 2620 675 
Q 2931 909 2931 1356 
Q 2931 1769 2642 2001 
Q 2353 2234 1838 2234 
L 1294 2234 
L 1294 2753 
L 1863 2753 
Q 2328 2753 2575 2939 
Q 2822 3125 2822 3475 
Q 2822 3834 2567 4026 
Q 2313 4219 1838 4219 
Q 1578 4219 1281 4162 
Q 984 4106 628 3988 
L 628 4550 
Q 988 4650 1302 4700 
Q 1616 4750 1894 4750 
Q 2613 4750 3031 4423 
Q 3450 4097 3450 3541 
Q 3450 3153 3228 2886 
Q 3006 2619 2597 2516 
z
" id="DejaVuSans-33" transform="scale(0.015625)"/>
       </defs>
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-33"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="ytick_2">
     <g id="line2d_11">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m09ba2c1beb" y="297.134122"/>
      </g>
     </g>
     <g id="text_12">
      <!-- $\mathdefault{10^{-25}}$ -->
      <g transform="translate(23.15 302.832951)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="ytick_3">
     <g id="line2d_12">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m09ba2c1beb" y="253.173054"/>
      </g>
     </g>
     <g id="text_13">
      <!-- $\mathdefault{10^{-20}}$ -->
      <g transform="translate(23.15 258.871882)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="ytick_4">
     <g id="line2d_13">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m09ba2c1beb" y="209.211986"/>
      </g>
     </g>
     <g id="text_14">
      <!-- $\mathdefault{10^{-15}}$ -->
      <g transform="translate(23.15 214.910814)scale(0.15 -0.15)">
       <use transform="translate(0 0.684375)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.684375)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 38.965625)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 38.965625)scale(0.7)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(231.391602 38.965625)scale(0.7)" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="ytick_5">
     <g id="line2d_14">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m09ba2c1beb" y="165.250917"/>
      </g>
     </g>
     <g id="text_15">
      <!-- $\mathdefault{10^{-10}}$ -->
      <g transform="translate(23.15 170.949745)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="ytick_6">
     <g id="line2d_15">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m09ba2c1beb" y="121.289849"/>
      </g>
     </g>
     <g id="text_16">
      <!-- $\mathdefault{10^{-5}}$ -->
      <g transform="translate(29.75 126.988677)scale(0.15 -0.15)">
       <use transform="translate(0 0.684375)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.684375)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 38.965625)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 38.965625)scale(0.7)" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="ytick_7">
     <g id="line2d_16">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#m09ba2c1beb" y="77.32878"/>
      </g>
     </g>
     <g id="text_17">
      <!-- $\mathdefault{10^{0}}$ -->
      <g transform="translate(38.6 83.027608)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="text_18">
     <!-- $||c_k-c*||^2$ -->
     <g transform="translate(15.55 256.02)rotate(-90)scale(0.15 -0.15)">
      <defs>
       <path d="M 1344 4891 
L 1344 -1509 
L 813 -1509 
L 813 4891 
L 1344 4891 
z
" id="DejaVuSans-7c" transform="scale(0.015625)"/>
       <path d="M 3431 3366 
L 3316 2797 
Q 3109 2947 2876 3022 
Q 2644 3097 2394 3097 
Q 2119 3097 1870 3000 
Q 1622 2903 1453 2725 
Q 1184 2453 1037 2087 
Q 891 1722 891 1331 
Q 891 859 1127 628 
Q 1363 397 1844 397 
Q 2081 397 2348 469 
Q 2616 541 2906 684 
L 2797 116 
Q 2547 13 2283 -39 
Q 2019 -91 1741 -91 
Q 1044 -91 669 257 
Q 294 606 294 1253 
Q 294 1797 489 2255 
Q 684 2713 1069 3078 
Q 1331 3328 1684 3456 
Q 2038 3584 2456 3584 
Q 2700 3584 2940 3529 
Q 3181 3475 3431 3366 
z
" id="DejaVuSans-Oblique-63" transform="scale(0.015625)"/>
       <path d="M 3009 3897 
L 1888 3291 
L 3009 2681 
L 2828 2375 
L 1778 3009 
L 1778 1831 
L 1422 1831 
L 1422 3009 
L 372 2375 
L 191 2681 
L 1313 3291 
L 191 3897 
L 372 4206 
L 1422 3572 
L 1422 4750 
L 1778 4750 
L 1778 3572 
L 2828 4206 
L 3009 3897 
z
" id="DejaVuSans-2a" transform="scale(0.015625)"/>
      </defs>
      <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(33.691406 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(67.382812 0.765625)" xlink:href="#DejaVuSans-Oblique-63"/>
      <use transform="translate(122.363281 -15.640625)scale(0.7)" xlink:href="#DejaVuSans-Oblique-6b"/>
      <use transform="translate(185.117188 0.765625)" xlink:href="#DejaVuSans-2212"/>
      <use transform="translate(288.388672 0.765625)" xlink:href="#DejaVuSans-Oblique-63"/>
      <use transform="translate(362.851562 0.765625)" xlink:href="#DejaVuSans-2a"/>
      <use transform="translate(432.333984 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(466.025391 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(500.673828 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
     </g>
    </g>
   </g>
   <g id="line2d_17">
    <path clip-path="url(#p6e77d7c011)" d="M 92.290909 66.687451 
L 94.330196 66.835866 
L 104.526633 66.925722 
L 126.958794 67.488734 
L 133.076656 67.660656 
L 151.430242 68.025285 
L 182.019552 68.45953 
L 184.05884 68.649325 
L 196.294564 68.771343 
L 200.373138 68.908407 
L 206.491 69.06285 
L 224.844587 69.428499 
L 228.923161 69.49464 
L 233.001736 69.561146 
L 239.119598 69.829504 
L 241.158885 70.041996 
L 261.551759 70.207811 
L 263.591046 70.347419 
L 273.787483 70.416113 
L 279.905345 70.469015 
L 288.062494 70.478499 
L 290.101782 70.643743 
L 304.376793 70.893639 
L 308.455368 71.089243 
L 326.808954 71.376893 
L 330.887529 71.502679 
L 341.083965 71.618892 
L 343.123253 71.783508 
L 347.201827 71.899245 
L 349.241115 72.034857 
L 359.437551 72.146999 
L 361.476839 72.381114 
L 367.594701 72.612267 
L 371.673275 72.68494 
L 381.869712 72.821409 
L 392.066149 73.057189 
L 400.223298 73.160796 
L 410.419735 73.386821 
L 414.49831 73.470084 
L 420.616172 73.634995 
L 434.891183 73.697325 
L 438.969758 73.786095 
L 447.126907 73.902978 
L 449.166195 73.940544 
L 453.244769 74.424016 
L 457.323344 74.556261 
L 469.559068 74.615619 
L 491.991229 74.72977 
L 494.030516 74.740237 
L 498.109091 75.224602 
L 498.109091 75.224602 
" style="fill:none;stroke:#0000ff;stroke-linecap:square;stroke-width:3;"/>
   </g>
   <g id="line2d_18">
    <path clip-path="url(#p6e77d7c011)" d="M 92.290909 68.789329 
L 94.330196 70.508019 
L 96.369484 73.259154 
L 98.408771 75.044986 
L 100.448058 76.336069 
L 102.487346 78.685523 
L 106.565921 82.846614 
L 108.605208 83.201042 
L 110.644495 85.413176 
L 114.72307 88.416007 
L 116.762357 90.620637 
L 118.801645 91.817228 
L 120.840932 91.996133 
L 122.880219 93.42971 
L 124.919507 95.945408 
L 126.958794 96.85166 
L 128.998081 97.526983 
L 131.037369 100.530344 
L 133.076656 101.660839 
L 135.115943 104.39262 
L 137.155231 106.73037 
L 139.194518 108.693927 
L 143.273093 111.585467 
L 145.31238 111.923779 
L 147.351667 115.496451 
L 151.430242 118.137897 
L 153.469529 118.588966 
L 155.508817 120.865165 
L 159.587392 124.81015 
L 161.626679 127.610179 
L 163.665966 129.553319 
L 165.705254 131.173512 
L 167.744541 133.521012 
L 169.783828 135.085885 
L 173.862403 138.852534 
L 175.90169 141.238546 
L 177.940978 143.398459 
L 179.980265 144.457336 
L 182.019552 144.759127 
L 184.05884 146.869364 
L 186.098127 147.423029 
L 188.137414 147.506956 
L 190.176702 148.470784 
L 192.215989 151.057287 
L 194.255276 153.330484 
L 200.373138 160.748336 
L 202.412426 162.482378 
L 204.451713 163.172924 
L 206.491 165.006402 
L 208.530288 167.376137 
L 210.569575 168.697214 
L 212.608862 169.79132 
L 214.64815 172.696831 
L 216.687437 172.810243 
L 218.726725 175.101273 
L 220.766012 175.110116 
L 222.805299 177.375853 
L 224.844587 177.442299 
L 226.883874 178.033788 
L 228.923161 179.725923 
L 230.962449 182.807648 
L 233.001736 184.455248 
L 235.041023 187.492779 
L 237.080311 189.811514 
L 239.119598 190.042996 
L 241.158885 191.91183 
L 243.198173 194.718927 
L 245.23746 195.864091 
L 247.276747 199.012799 
L 249.316035 199.311885 
L 251.355322 201.304549 
L 253.394609 204.420681 
L 255.433897 206.812345 
L 257.473184 207.174181 
L 261.551759 210.645189 
L 263.591046 212.664486 
L 265.630333 215.40793 
L 267.669621 217.871825 
L 269.708908 219.189098 
L 271.748196 221.64416 
L 273.787483 223.563351 
L 275.82677 225.845675 
L 277.866058 229.159716 
L 279.905345 232.239029 
L 281.944632 235.078229 
L 283.98392 236.846489 
L 286.023207 238.833512 
L 288.062494 238.874444 
L 290.101782 240.30172 
L 292.141069 240.316212 
L 296.219644 244.324181 
L 298.258931 245.180601 
L 300.298218 247.135997 
L 302.337506 248.697515 
L 304.376793 250.709117 
L 306.41608 253.053899 
L 308.455368 254.537948 
L 312.533942 256.721051 
L 318.651804 263.279817 
L 320.691092 264.260763 
L 322.730379 265.826585 
L 324.769667 268.719337 
L 326.808954 271.034459 
L 330.887529 276.861342 
L 332.926816 277.491193 
L 334.966103 279.111818 
L 337.005391 281.24747 
L 339.044678 283.084028 
L 341.083965 285.647783 
L 343.123253 285.904473 
L 345.16254 285.913812 
L 347.201827 288.146759 
L 349.241115 289.781873 
L 353.319689 294.063401 
L 355.358977 294.821208 
L 357.398264 296.685323 
L 359.437551 300.066473 
L 361.476839 302.83584 
L 363.516126 305.12133 
L 365.555413 306.559338 
L 371.673275 312.656698 
L 373.712563 313.840391 
L 375.75185 314.252633 
L 379.830425 314.611823 
L 381.869712 317.215592 
L 383.909 318.407243 
L 385.948287 321.221729 
L 387.987574 321.765017 
L 390.026862 324.039835 
L 394.105436 329.224686 
L 398.184011 331.237205 
L 404.301873 338.07354 
L 406.34116 340.730941 
L 412.459022 346.035092 
L 414.49831 346.035092 
L 416.537597 346.791813 
L 418.576884 347.872905 
L 420.616172 348.724958 
L 428.773321 348.724958 
L 430.812608 349.088892 
L 432.851896 349.185565 
L 434.891183 349.598769 
L 438.969758 349.598769 
L 441.009045 350.883558 
L 445.08762 350.883558 
L 447.126907 352.137921 
L 449.166195 352.137921 
L 451.205482 352.356176 
L 453.244769 355.744263 
L 457.323344 357.029052 
L 459.362631 357.029052 
L 461.401919 357.881105 
L 465.480493 357.881105 
L 467.519781 358.979593 
L 477.716217 358.979593 
L 479.755505 360.527825 
L 491.991229 360.527825 
L 494.030516 363.174545 
L 498.109091 363.174545 
L 498.109091 363.174545 
" style="fill:none;stroke:#008000;stroke-dasharray:11.1,4.8;stroke-dashoffset:0;stroke-width:3;"/>
   </g>
   <g id="line2d_19">
    <path clip-path="url(#p6e77d7c011)" d="M 92.290909 66.665455 
L 98.408771 67.079972 
L 102.487346 67.554633 
L 108.605208 68.01926 
L 114.72307 68.809691 
L 118.801645 69.043331 
L 120.840932 69.267683 
L 124.919507 69.469733 
L 126.958794 69.751604 
L 133.076656 69.979873 
L 135.115943 70.321375 
L 137.155231 70.81582 
L 141.233805 71.025536 
L 143.273093 71.425777 
L 151.430242 72.154019 
L 153.469529 72.502975 
L 155.508817 72.972833 
L 163.665966 73.47959 
L 165.705254 73.936286 
L 169.783828 74.151153 
L 171.823116 74.671296 
L 175.90169 74.808555 
L 177.940978 75.26861 
L 184.05884 75.564254 
L 186.098127 76.619484 
L 198.333851 77.158018 
L 200.373138 78.859605 
L 202.412426 79.300609 
L 204.451713 79.344644 
L 208.530288 79.704376 
L 212.608862 79.81512 
L 216.687437 79.998547 
L 220.766012 80.062735 
L 222.805299 80.347579 
L 255.433897 81.521809 
L 257.473184 81.876219 
L 261.551759 82.216751 
L 265.630333 82.305841 
L 267.669621 82.46264 
L 279.905345 82.600305 
L 281.944632 83.070916 
L 286.023207 83.157316 
L 294.180356 83.324685 
L 296.219644 83.380819 
L 298.258931 85.022379 
L 302.337506 85.170022 
L 306.41608 85.205451 
L 308.455368 85.563233 
L 318.651804 85.649198 
L 320.691092 88.890679 
L 324.769667 89.022685 
L 328.848241 89.047036 
L 330.887529 89.308882 
L 332.926816 89.419993 
L 334.966103 90.344002 
L 339.044678 90.484264 
L 343.123253 90.59534 
L 349.241115 90.70141 
L 359.437551 90.818168 
L 361.476839 91.198321 
L 371.673275 91.329864 
L 381.869712 91.6587 
L 383.909 92.167594 
L 387.987574 92.295144 
L 400.223298 92.477484 
L 402.262586 97.654247 
L 416.537597 98.317658 
L 420.616172 99.712275 
L 422.655459 99.722793 
L 424.694746 99.897165 
L 434.891183 100.155449 
L 438.969758 101.912339 
L 441.009045 102.346127 
L 447.126907 102.524997 
L 449.166195 102.627329 
L 451.205482 103.555107 
L 455.284057 103.738588 
L 457.323344 104.30018 
L 461.401919 104.632514 
L 465.480493 104.726678 
L 469.559068 104.860337 
L 471.598355 105.431059 
L 475.67693 105.958518 
L 498.109091 106.452327 
L 498.109091 106.452327 
" style="fill:none;stroke:#ff0000;stroke-dasharray:3,4.95;stroke-dashoffset:0;stroke-width:3;"/>
   </g>
   <g id="line2d_20">
    <path clip-path="url(#p6e77d7c011)" d="M 92.290909 67.058186 
L 102.487346 69.033136 
L 106.565921 69.731724 
L 112.683783 71.104582 
L 114.72307 71.200173 
L 116.762357 71.513157 
L 118.801645 71.657744 
L 120.840932 71.958512 
L 124.919507 72.054312 
L 126.958794 72.11292 
L 128.998081 72.545926 
L 131.037369 72.772619 
L 133.076656 73.210893 
L 139.194518 74.207394 
L 151.430242 76.741412 
L 161.626679 78.223085 
L 163.665966 78.410384 
L 165.705254 78.926524 
L 167.744541 79.29826 
L 169.783828 80.021415 
L 171.823116 80.320332 
L 173.862403 80.395623 
L 175.90169 81.00069 
L 177.940978 81.296799 
L 179.980265 81.339889 
L 182.019552 81.568031 
L 184.05884 82.043849 
L 188.137414 82.335739 
L 190.176702 83.122164 
L 192.215989 83.591725 
L 194.255276 84.203951 
L 198.333851 84.967948 
L 204.451713 85.275303 
L 206.491 85.736017 
L 212.608862 86.655326 
L 214.64815 86.738777 
L 216.687437 86.990565 
L 218.726725 87.030415 
L 226.883874 87.841635 
L 228.923161 88.429447 
L 230.962449 88.552654 
L 233.001736 89.143268 
L 235.041023 90.266533 
L 237.080311 90.744725 
L 241.158885 91.339778 
L 243.198173 91.592185 
L 245.23746 92.094732 
L 247.276747 92.25342 
L 251.355322 92.726576 
L 253.394609 93.234719 
L 257.473184 93.759666 
L 259.512471 93.88309 
L 261.551759 94.28083 
L 267.669621 94.725285 
L 273.787483 95.512453 
L 275.82677 95.640377 
L 277.866058 96.003811 
L 290.101782 97.383747 
L 292.141069 97.442416 
L 302.337506 98.875662 
L 304.376793 98.9391 
L 306.41608 99.984663 
L 308.455368 100.454369 
L 310.494655 100.690831 
L 312.533942 100.701886 
L 318.651804 101.172627 
L 320.691092 101.858264 
L 322.730379 101.858264 
L 330.887529 102.295355 
L 334.966103 102.369673 
L 337.005391 103.205781 
L 349.241115 104.778613 
L 351.280402 105.021431 
L 357.398264 105.321746 
L 359.437551 105.960533 
L 361.476839 106.200417 
L 363.516126 106.627841 
L 367.594701 107.076197 
L 369.633988 107.101515 
L 371.673275 107.456714 
L 373.712563 107.954276 
L 375.75185 108.031433 
L 377.791138 108.232259 
L 381.869712 108.266438 
L 390.026862 109.121559 
L 392.066149 109.903987 
L 394.105436 110.049355 
L 396.144724 110.521177 
L 398.184011 111.122171 
L 400.223298 111.349514 
L 408.380448 111.547105 
L 410.419735 111.763515 
L 412.459022 112.282645 
L 414.49831 112.378303 
L 416.537597 112.643912 
L 418.576884 112.659066 
L 422.655459 113.069578 
L 430.812608 113.984418 
L 432.851896 114.01584 
L 436.930471 114.70296 
L 451.205482 115.395086 
L 455.284057 115.879265 
L 457.323344 116.262637 
L 459.362631 116.33439 
L 461.401919 116.662525 
L 475.67693 117.306208 
L 477.716217 119.042392 
L 481.794792 119.196268 
L 483.834079 120.150667 
L 485.873367 120.29891 
L 487.912654 120.997719 
L 489.951942 121.083808 
L 491.991229 121.345049 
L 498.109091 121.583265 
L 498.109091 121.583265 
" style="fill:none;stroke:#1f77b4;stroke-dasharray:19.2,4.8,3,4.8;stroke-dashoffset:0;stroke-width:3;"/>
    <defs>
     <path d="M 0 -3 
L -2.85317 -0.927051 
L -1.763356 2.427051 
L 1.763356 2.427051 
L 2.85317 -0.927051 
z
" id="m6ba5757cde" style="stroke:#1f77b4;stroke-linejoin:miter;"/>
    </defs>
    <g clip-path="url(#p6e77d7c011)">
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="92.290909" xlink:href="#m6ba5757cde" y="67.058186"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="94.330196" xlink:href="#m6ba5757cde" y="67.464107"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="96.369484" xlink:href="#m6ba5757cde" y="67.965747"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="98.408771" xlink:href="#m6ba5757cde" y="68.32709"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="100.448058" xlink:href="#m6ba5757cde" y="68.592669"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="102.487346" xlink:href="#m6ba5757cde" y="69.033136"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="104.526633" xlink:href="#m6ba5757cde" y="69.33396"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="106.565921" xlink:href="#m6ba5757cde" y="69.731724"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="108.605208" xlink:href="#m6ba5757cde" y="70.161242"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="110.644495" xlink:href="#m6ba5757cde" y="70.625331"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="112.683783" xlink:href="#m6ba5757cde" y="71.104582"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="114.72307" xlink:href="#m6ba5757cde" y="71.200173"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="116.762357" xlink:href="#m6ba5757cde" y="71.513157"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="118.801645" xlink:href="#m6ba5757cde" y="71.657744"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="120.840932" xlink:href="#m6ba5757cde" y="71.958512"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="122.880219" xlink:href="#m6ba5757cde" y="72.047457"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="124.919507" xlink:href="#m6ba5757cde" y="72.054312"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="126.958794" xlink:href="#m6ba5757cde" y="72.11292"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="128.998081" xlink:href="#m6ba5757cde" y="72.545926"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="131.037369" xlink:href="#m6ba5757cde" y="72.772619"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="133.076656" xlink:href="#m6ba5757cde" y="73.210893"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="135.115943" xlink:href="#m6ba5757cde" y="73.518399"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="137.155231" xlink:href="#m6ba5757cde" y="73.760941"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="139.194518" xlink:href="#m6ba5757cde" y="74.207394"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="141.233805" xlink:href="#m6ba5757cde" y="74.641584"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="143.273093" xlink:href="#m6ba5757cde" y="75.069535"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="145.31238" xlink:href="#m6ba5757cde" y="75.449901"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="147.351667" xlink:href="#m6ba5757cde" y="75.88968"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="149.390955" xlink:href="#m6ba5757cde" y="76.444634"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="151.430242" xlink:href="#m6ba5757cde" y="76.741412"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="153.469529" xlink:href="#m6ba5757cde" y="77.058248"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="155.508817" xlink:href="#m6ba5757cde" y="77.346771"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="157.548104" xlink:href="#m6ba5757cde" y="77.691942"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="159.587392" xlink:href="#m6ba5757cde" y="78.074485"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="161.626679" xlink:href="#m6ba5757cde" y="78.223085"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="163.665966" xlink:href="#m6ba5757cde" y="78.410384"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="165.705254" xlink:href="#m6ba5757cde" y="78.926524"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="167.744541" xlink:href="#m6ba5757cde" y="79.29826"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="169.783828" xlink:href="#m6ba5757cde" y="80.021415"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="171.823116" xlink:href="#m6ba5757cde" y="80.320332"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="173.862403" xlink:href="#m6ba5757cde" y="80.395623"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="175.90169" xlink:href="#m6ba5757cde" y="81.00069"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="177.940978" xlink:href="#m6ba5757cde" y="81.296799"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="179.980265" xlink:href="#m6ba5757cde" y="81.339889"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="182.019552" xlink:href="#m6ba5757cde" y="81.568031"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="184.05884" xlink:href="#m6ba5757cde" y="82.043849"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="186.098127" xlink:href="#m6ba5757cde" y="82.237387"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="188.137414" xlink:href="#m6ba5757cde" y="82.335739"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="190.176702" xlink:href="#m6ba5757cde" y="83.122164"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="192.215989" xlink:href="#m6ba5757cde" y="83.591725"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="194.255276" xlink:href="#m6ba5757cde" y="84.203951"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="196.294564" xlink:href="#m6ba5757cde" y="84.639787"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="198.333851" xlink:href="#m6ba5757cde" y="84.967948"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="200.373138" xlink:href="#m6ba5757cde" y="85.09092"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="202.412426" xlink:href="#m6ba5757cde" y="85.275303"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="204.451713" xlink:href="#m6ba5757cde" y="85.275303"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="206.491" xlink:href="#m6ba5757cde" y="85.736017"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="208.530288" xlink:href="#m6ba5757cde" y="86.071008"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="210.569575" xlink:href="#m6ba5757cde" y="86.423687"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="212.608862" xlink:href="#m6ba5757cde" y="86.655326"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="214.64815" xlink:href="#m6ba5757cde" y="86.738777"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="216.687437" xlink:href="#m6ba5757cde" y="86.990565"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="218.726725" xlink:href="#m6ba5757cde" y="87.030415"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="220.766012" xlink:href="#m6ba5757cde" y="87.223134"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="222.805299" xlink:href="#m6ba5757cde" y="87.514409"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="224.844587" xlink:href="#m6ba5757cde" y="87.530957"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="226.883874" xlink:href="#m6ba5757cde" y="87.841635"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="228.923161" xlink:href="#m6ba5757cde" y="88.429447"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="230.962449" xlink:href="#m6ba5757cde" y="88.552654"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="233.001736" xlink:href="#m6ba5757cde" y="89.143268"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="235.041023" xlink:href="#m6ba5757cde" y="90.266533"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="237.080311" xlink:href="#m6ba5757cde" y="90.744725"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="239.119598" xlink:href="#m6ba5757cde" y="91.068659"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="241.158885" xlink:href="#m6ba5757cde" y="91.339778"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="243.198173" xlink:href="#m6ba5757cde" y="91.592185"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="245.23746" xlink:href="#m6ba5757cde" y="92.094732"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="247.276747" xlink:href="#m6ba5757cde" y="92.25342"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="249.316035" xlink:href="#m6ba5757cde" y="92.527138"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="251.355322" xlink:href="#m6ba5757cde" y="92.726576"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="253.394609" xlink:href="#m6ba5757cde" y="93.234719"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="255.433897" xlink:href="#m6ba5757cde" y="93.507728"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="257.473184" xlink:href="#m6ba5757cde" y="93.759666"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="259.512471" xlink:href="#m6ba5757cde" y="93.88309"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="261.551759" xlink:href="#m6ba5757cde" y="94.28083"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="263.591046" xlink:href="#m6ba5757cde" y="94.405224"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="265.630333" xlink:href="#m6ba5757cde" y="94.60966"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="267.669621" xlink:href="#m6ba5757cde" y="94.725285"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="269.708908" xlink:href="#m6ba5757cde" y="95.017631"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="271.748196" xlink:href="#m6ba5757cde" y="95.311903"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="273.787483" xlink:href="#m6ba5757cde" y="95.512453"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="275.82677" xlink:href="#m6ba5757cde" y="95.640377"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="277.866058" xlink:href="#m6ba5757cde" y="96.003811"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="279.905345" xlink:href="#m6ba5757cde" y="96.225616"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="281.944632" xlink:href="#m6ba5757cde" y="96.388509"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="283.98392" xlink:href="#m6ba5757cde" y="96.71081"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="286.023207" xlink:href="#m6ba5757cde" y="96.903747"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="288.062494" xlink:href="#m6ba5757cde" y="97.040972"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="290.101782" xlink:href="#m6ba5757cde" y="97.383747"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="292.141069" xlink:href="#m6ba5757cde" y="97.442416"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="294.180356" xlink:href="#m6ba5757cde" y="97.735135"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="296.219644" xlink:href="#m6ba5757cde" y="97.98162"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="298.258931" xlink:href="#m6ba5757cde" y="98.245"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="300.298218" xlink:href="#m6ba5757cde" y="98.560019"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="302.337506" xlink:href="#m6ba5757cde" y="98.875662"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="304.376793" xlink:href="#m6ba5757cde" y="98.9391"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="306.41608" xlink:href="#m6ba5757cde" y="99.984663"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="308.455368" xlink:href="#m6ba5757cde" y="100.454369"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="310.494655" xlink:href="#m6ba5757cde" y="100.690831"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="312.533942" xlink:href="#m6ba5757cde" y="100.701886"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="314.57323" xlink:href="#m6ba5757cde" y="100.841674"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="316.612517" xlink:href="#m6ba5757cde" y="101.020036"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="318.651804" xlink:href="#m6ba5757cde" y="101.172627"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="320.691092" xlink:href="#m6ba5757cde" y="101.858264"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="322.730379" xlink:href="#m6ba5757cde" y="101.858264"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="324.769667" xlink:href="#m6ba5757cde" y="101.973922"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="326.808954" xlink:href="#m6ba5757cde" y="102.064487"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="328.848241" xlink:href="#m6ba5757cde" y="102.138904"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="330.887529" xlink:href="#m6ba5757cde" y="102.295355"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="332.926816" xlink:href="#m6ba5757cde" y="102.305081"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="334.966103" xlink:href="#m6ba5757cde" y="102.369673"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="337.005391" xlink:href="#m6ba5757cde" y="103.205781"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="339.044678" xlink:href="#m6ba5757cde" y="103.485779"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="341.083965" xlink:href="#m6ba5757cde" y="103.779186"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="343.123253" xlink:href="#m6ba5757cde" y="104.143225"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="345.16254" xlink:href="#m6ba5757cde" y="104.351096"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="347.201827" xlink:href="#m6ba5757cde" y="104.612159"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="349.241115" xlink:href="#m6ba5757cde" y="104.778613"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="351.280402" xlink:href="#m6ba5757cde" y="105.021431"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="353.319689" xlink:href="#m6ba5757cde" y="105.127826"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="355.358977" xlink:href="#m6ba5757cde" y="105.193067"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="357.398264" xlink:href="#m6ba5757cde" y="105.321746"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="359.437551" xlink:href="#m6ba5757cde" y="105.960533"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="361.476839" xlink:href="#m6ba5757cde" y="106.200417"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="363.516126" xlink:href="#m6ba5757cde" y="106.627841"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="365.555413" xlink:href="#m6ba5757cde" y="106.831073"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="367.594701" xlink:href="#m6ba5757cde" y="107.076197"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="369.633988" xlink:href="#m6ba5757cde" y="107.101515"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="371.673275" xlink:href="#m6ba5757cde" y="107.456714"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="373.712563" xlink:href="#m6ba5757cde" y="107.954276"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="375.75185" xlink:href="#m6ba5757cde" y="108.031433"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="377.791138" xlink:href="#m6ba5757cde" y="108.232259"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="379.830425" xlink:href="#m6ba5757cde" y="108.265036"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="381.869712" xlink:href="#m6ba5757cde" y="108.266438"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="383.909" xlink:href="#m6ba5757cde" y="108.470071"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="385.948287" xlink:href="#m6ba5757cde" y="108.688154"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="387.987574" xlink:href="#m6ba5757cde" y="108.802715"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="390.026862" xlink:href="#m6ba5757cde" y="109.121559"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="392.066149" xlink:href="#m6ba5757cde" y="109.903987"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="394.105436" xlink:href="#m6ba5757cde" y="110.049355"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="396.144724" xlink:href="#m6ba5757cde" y="110.521177"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="398.184011" xlink:href="#m6ba5757cde" y="111.122171"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="400.223298" xlink:href="#m6ba5757cde" y="111.349514"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="402.262586" xlink:href="#m6ba5757cde" y="111.392443"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="404.301873" xlink:href="#m6ba5757cde" y="111.45049"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="406.34116" xlink:href="#m6ba5757cde" y="111.460578"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="408.380448" xlink:href="#m6ba5757cde" y="111.547105"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="410.419735" xlink:href="#m6ba5757cde" y="111.763515"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="412.459022" xlink:href="#m6ba5757cde" y="112.282645"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="414.49831" xlink:href="#m6ba5757cde" y="112.378303"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="416.537597" xlink:href="#m6ba5757cde" y="112.643912"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="418.576884" xlink:href="#m6ba5757cde" y="112.659066"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="420.616172" xlink:href="#m6ba5757cde" y="112.810732"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="422.655459" xlink:href="#m6ba5757cde" y="113.069578"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="424.694746" xlink:href="#m6ba5757cde" y="113.289121"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="426.734034" xlink:href="#m6ba5757cde" y="113.501809"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="428.773321" xlink:href="#m6ba5757cde" y="113.704101"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="430.812608" xlink:href="#m6ba5757cde" y="113.984418"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="432.851896" xlink:href="#m6ba5757cde" y="114.01584"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="434.891183" xlink:href="#m6ba5757cde" y="114.40702"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="436.930471" xlink:href="#m6ba5757cde" y="114.70296"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="438.969758" xlink:href="#m6ba5757cde" y="114.799938"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="441.009045" xlink:href="#m6ba5757cde" y="114.854803"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="443.048333" xlink:href="#m6ba5757cde" y="114.894967"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="445.08762" xlink:href="#m6ba5757cde" y="115.15116"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="447.126907" xlink:href="#m6ba5757cde" y="115.209755"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="449.166195" xlink:href="#m6ba5757cde" y="115.283685"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="451.205482" xlink:href="#m6ba5757cde" y="115.395086"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="453.244769" xlink:href="#m6ba5757cde" y="115.609803"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="455.284057" xlink:href="#m6ba5757cde" y="115.879265"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="457.323344" xlink:href="#m6ba5757cde" y="116.262637"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="459.362631" xlink:href="#m6ba5757cde" y="116.33439"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="461.401919" xlink:href="#m6ba5757cde" y="116.662525"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="463.441206" xlink:href="#m6ba5757cde" y="116.759483"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="465.480493" xlink:href="#m6ba5757cde" y="116.955604"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="467.519781" xlink:href="#m6ba5757cde" y="117.04165"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="469.559068" xlink:href="#m6ba5757cde" y="117.096252"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="471.598355" xlink:href="#m6ba5757cde" y="117.185571"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="473.637643" xlink:href="#m6ba5757cde" y="117.234892"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="475.67693" xlink:href="#m6ba5757cde" y="117.306208"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="477.716217" xlink:href="#m6ba5757cde" y="119.042392"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="479.755505" xlink:href="#m6ba5757cde" y="119.077384"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="481.794792" xlink:href="#m6ba5757cde" y="119.196268"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="483.834079" xlink:href="#m6ba5757cde" y="120.150667"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="485.873367" xlink:href="#m6ba5757cde" y="120.29891"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="487.912654" xlink:href="#m6ba5757cde" y="120.997719"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="489.951942" xlink:href="#m6ba5757cde" y="121.083808"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="491.991229" xlink:href="#m6ba5757cde" y="121.345049"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="494.030516" xlink:href="#m6ba5757cde" y="121.421773"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="496.069804" xlink:href="#m6ba5757cde" y="121.490075"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="498.109091" xlink:href="#m6ba5757cde" y="121.583265"/>
    </g>
   </g>
   <g id="patch_3">
    <path d="M 72 378 
L 72 51.84 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="patch_4">
    <path d="M 518.4 378 
L 518.4 51.84 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="patch_5">
    <path d="M 72 378 
L 518.4 378 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="patch_6">
    <path d="M 72 51.84 
L 518.4 51.84 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="legend_1">
    <g id="patch_7">
     <path d="M 82.5 370.5 
L 176.446875 370.5 
Q 179.446875 370.5 179.446875 367.5 
L 179.446875 280.93125 
Q 179.446875 277.93125 176.446875 277.93125 
L 82.5 277.93125 
Q 79.5 277.93125 79.5 280.93125 
L 79.5 367.5 
Q 79.5 370.5 82.5 370.5 
z
" style="fill:#ffffff;opacity:0.8;stroke:#cccccc;stroke-linejoin:miter;"/>
    </g>
    <g id="line2d_21">
     <path d="M 85.5 290.078906 
L 115.5 290.078906 
" style="fill:none;stroke:#0000ff;stroke-linecap:square;stroke-width:3;"/>
    </g>
    <g id="line2d_22"/>
    <g id="text_19">
     <!-- p=0.2 -->
     <g transform="translate(127.5 295.328906)scale(0.15 -0.15)">
      <defs>
       <path d="M 1159 525 
L 1159 -1331 
L 581 -1331 
L 581 3500 
L 1159 3500 
L 1159 2969 
Q 1341 3281 1617 3432 
Q 1894 3584 2278 3584 
Q 2916 3584 3314 3078 
Q 3713 2572 3713 1747 
Q 3713 922 3314 415 
Q 2916 -91 2278 -91 
Q 1894 -91 1617 61 
Q 1341 213 1159 525 
z
M 3116 1747 
Q 3116 2381 2855 2742 
Q 2594 3103 2138 3103 
Q 1681 3103 1420 2742 
Q 1159 2381 1159 1747 
Q 1159 1113 1420 752 
Q 1681 391 2138 391 
Q 2594 391 2855 752 
Q 3116 1113 3116 1747 
z
" id="DejaVuSans-70" transform="scale(0.015625)"/>
       <path d="M 678 2906 
L 4684 2906 
L 4684 2381 
L 678 2381 
L 678 2906 
z
M 678 1631 
L 4684 1631 
L 4684 1100 
L 678 1100 
L 678 1631 
z
" id="DejaVuSans-3d" transform="scale(0.015625)"/>
       <path d="M 684 794 
L 1344 794 
L 1344 0 
L 684 0 
L 684 794 
z
" id="DejaVuSans-2e" transform="scale(0.015625)"/>
      </defs>
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-30"/>
      <use x="210.888672" xlink:href="#DejaVuSans-2e"/>
      <use x="242.675781" xlink:href="#DejaVuSans-32"/>
     </g>
    </g>
    <g id="line2d_23">
     <path d="M 85.5 312.096094 
L 115.5 312.096094 
" style="fill:none;stroke:#008000;stroke-dasharray:11.1,4.8;stroke-dashoffset:0;stroke-width:3;"/>
    </g>
    <g id="line2d_24"/>
    <g id="text_20">
     <!-- p=0.4 -->
     <g transform="translate(127.5 317.346094)scale(0.15 -0.15)">
      <defs>
       <path d="M 2419 4116 
L 825 1625 
L 2419 1625 
L 2419 4116 
z
M 2253 4666 
L 3047 4666 
L 3047 1625 
L 3713 1625 
L 3713 1100 
L 3047 1100 
L 3047 0 
L 2419 0 
L 2419 1100 
L 313 1100 
L 313 1709 
L 2253 4666 
z
" id="DejaVuSans-34" transform="scale(0.015625)"/>
      </defs>
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-30"/>
      <use x="210.888672" xlink:href="#DejaVuSans-2e"/>
      <use x="242.675781" xlink:href="#DejaVuSans-34"/>
     </g>
    </g>
    <g id="line2d_25">
     <path d="M 85.5 334.113281 
L 115.5 334.113281 
" style="fill:none;stroke:#ff0000;stroke-dasharray:3,4.95;stroke-dashoffset:0;stroke-width:3;"/>
    </g>
    <g id="line2d_26"/>
    <g id="text_21">
     <!-- p=0.6 -->
     <g transform="translate(127.5 339.363281)scale(0.15 -0.15)">
      <defs>
       <path d="M 2113 2584 
Q 1688 2584 1439 2293 
Q 1191 2003 1191 1497 
Q 1191 994 1439 701 
Q 1688 409 2113 409 
Q 2538 409 2786 701 
Q 3034 994 3034 1497 
Q 3034 2003 2786 2293 
Q 2538 2584 2113 2584 
z
M 3366 4563 
L 3366 3988 
Q 3128 4100 2886 4159 
Q 2644 4219 2406 4219 
Q 1781 4219 1451 3797 
Q 1122 3375 1075 2522 
Q 1259 2794 1537 2939 
Q 1816 3084 2150 3084 
Q 2853 3084 3261 2657 
Q 3669 2231 3669 1497 
Q 3669 778 3244 343 
Q 2819 -91 2113 -91 
Q 1303 -91 875 529 
Q 447 1150 447 2328 
Q 447 3434 972 4092 
Q 1497 4750 2381 4750 
Q 2619 4750 2861 4703 
Q 3103 4656 3366 4563 
z
" id="DejaVuSans-36" transform="scale(0.015625)"/>
      </defs>
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-30"/>
      <use x="210.888672" xlink:href="#DejaVuSans-2e"/>
      <use x="242.675781" xlink:href="#DejaVuSans-36"/>
     </g>
    </g>
    <g id="line2d_27">
     <path d="M 85.5 356.130469 
L 115.5 356.130469 
" style="fill:none;stroke:#1f77b4;stroke-dasharray:19.2,4.8,3,4.8;stroke-dashoffset:0;stroke-width:3;"/>
    </g>
    <g id="line2d_28">
     <g>
      <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="100.5" xlink:href="#m6ba5757cde" y="356.130469"/>
     </g>
    </g>
    <g id="text_22">
     <!-- p=1 -->
     <g transform="translate(127.5 361.380469)scale(0.15 -0.15)">
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-31"/>
     </g>
    </g>
   </g>
  </g>
 </g>
 <defs>
  <clipPath id="p6e77d7c011">
   <rect height="326.16" width="446.4" x="72" y="51.84"/>
  </clipPath>
 </defs>
</svg>


==> figs/p06_all_methods <==
<?xml version="1.0" encoding="utf-8" standalone="no"?>
<!DOCTYPE svg PUBLIC "-//W3C//DTD SVG 1.1//EN"
  "http://www.w3.org/Graphics/SVG/1.1/DTD/svg11.dtd">
<svg height="432pt" version="1.1" viewBox="0 0 576 432" width="576pt" xmlns="http://www.w3.org/2000/svg" xmlns:xlink="http://www.w3.org/1999/xlink">
 <metadata>
  <rdf:RDF xmlns:cc="http://creativecommons.org/ns#" xmlns:dc="http://purl.org/dc/elements/1.1/" xmlns:rdf="http://www.w3.org/1999/02/22-rdf-syntax-ns#">
   <cc:Work>
    <dc:type rdf:resource="http://purl.org/dc/dcmitype/StillImage"/>
    <dc:date>2021-10-19T15:48:47.458469</dc:date>
    <dc:format>image/svg+xml</dc:format>
    <dc:creator>
     <cc:Agent>
      <dc:title>Matplotlib v3.4.2, https://matplotlib.org/</dc:title>
     </cc:Agent>
    </dc:creator>
   </cc:Work>
  </rdf:RDF>
 </metadata>
 <defs>
  <style type="text/css">*{stroke-linecap:butt;stroke-linejoin:round;}</style>
 </defs>
 <g id="figure_1">
  <g id="patch_1">
   <path d="M 0 432 
L 576 432 
L 576 0 
L 0 0 
z
" style="fill:none;"/>
  </g>
  <g id="axes_1">
   <g id="patch_2">
    <path d="M 72 378 
L 518.4 378 
L 518.4 51.84 
L 72 51.84 
z
" style="fill:#ffffff;"/>
   </g>
   <g id="matplotlib.axis_1">
    <g id="xtick_1">
     <g id="line2d_1">
      <defs>
       <path d="M 0 0 
L 0 3.5 
" id="m0a42397935" style="stroke:#000000;stroke-width:0.8;"/>
      </defs>
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="92.290909" xlink:href="#m0a42397935" y="378"/>
      </g>
     </g>
     <g id="text_1">
      <!-- 0 -->
      <g transform="translate(87.519034 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 2034 4250 
Q 1547 4250 1301 3770 
Q 1056 3291 1056 2328 
Q 1056 1369 1301 889 
Q 1547 409 2034 409 
Q 2525 409 2770 889 
Q 3016 1369 3016 2328 
Q 3016 3291 2770 3770 
Q 2525 4250 2034 4250 
z
M 2034 4750 
Q 2819 4750 3233 4129 
Q 3647 3509 3647 2328 
Q 3647 1150 3233 529 
Q 2819 -91 2034 -91 
Q 1250 -91 836 529 
Q 422 1150 422 2328 
Q 422 3509 836 4129 
Q 1250 4750 2034 4750 
z
" id="DejaVuSans-30" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_2">
     <g id="line2d_2">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="143.273093" xlink:href="#m0a42397935" y="378"/>
      </g>
     </g>
     <g id="text_2">
      <!-- 25 -->
      <g transform="translate(133.729343 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 1228 531 
L 3431 531 
L 3431 0 
L 469 0 
L 469 531 
Q 828 903 1448 1529 
Q 2069 2156 2228 2338 
Q 2531 2678 2651 2914 
Q 2772 3150 2772 3378 
Q 2772 3750 2511 3984 
Q 2250 4219 1831 4219 
Q 1534 4219 1204 4116 
Q 875 4013 500 3803 
L 500 4441 
Q 881 4594 1212 4672 
Q 1544 4750 1819 4750 
Q 2544 4750 2975 4387 
Q 3406 4025 3406 3419 
Q 3406 3131 3298 2873 
Q 3191 2616 2906 2266 
Q 2828 2175 2409 1742 
Q 1991 1309 1228 531 
z
" id="DejaVuSans-32" transform="scale(0.015625)"/>
        <path d="M 691 4666 
L 3169 4666 
L 3169 4134 
L 1269 4134 
L 1269 2991 
Q 1406 3038 1543 3061 
Q 1681 3084 1819 3084 
Q 2600 3084 3056 2656 
Q 3513 2228 3513 1497 
Q 3513 744 3044 326 
Q 2575 -91 1722 -91 
Q 1428 -91 1123 -41 
Q 819 9 494 109 
L 494 744 
Q 775 591 1075 516 
Q 1375 441 1709 441 
Q 2250 441 2565 725 
Q 2881 1009 2881 1497 
Q 2881 1984 2565 2268 
Q 2250 2553 1709 2553 
Q 1456 2553 1204 2497 
Q 953 2441 691 2322 
L 691 4666 
z
" id="DejaVuSans-35" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-32"/>
       <use x="63.623047" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_3">
     <g id="line2d_3">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="194.255276" xlink:href="#m0a42397935" y="378"/>
      </g>
     </g>
     <g id="text_3">
      <!-- 50 -->
      <g transform="translate(184.711526 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-35"/>
       <use x="63.623047" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_4">
     <g id="line2d_4">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="245.23746" xlink:href="#m0a42397935" y="378"/>
      </g>
     </g>
     <g id="text_4">
      <!-- 75 -->
      <g transform="translate(235.69371 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 525 4666 
L 3525 4666 
L 3525 4397 
L 1831 0 
L 1172 0 
L 2766 4134 
L 525 4134 
L 525 4666 
z
" id="DejaVuSans-37" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-37"/>
       <use x="63.623047" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_5">
     <g id="line2d_5">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="296.219644" xlink:href="#m0a42397935" y="378"/>
      </g>
     </g>
     <g id="text_5">
      <!-- 100 -->
      <g transform="translate(281.904019 396.397656)scale(0.15 -0.15)">
       <defs>
        <path d="M 794 531 
L 1825 531 
L 1825 4091 
L 703 3866 
L 703 4441 
L 1819 4666 
L 2450 4666 
L 2450 531 
L 3481 531 
L 3481 0 
L 794 0 
L 794 531 
z
" id="DejaVuSans-31" transform="scale(0.015625)"/>
       </defs>
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-30"/>
       <use x="127.246094" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_6">
     <g id="line2d_6">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="347.201827" xlink:href="#m0a42397935" y="378"/>
      </g>
     </g>
     <g id="text_6">
      <!-- 125 -->
      <g transform="translate(332.886202 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-32"/>
       <use x="127.246094" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_7">
     <g id="line2d_7">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="398.184011" xlink:href="#m0a42397935" y="378"/>
      </g>
     </g>
     <g id="text_7">
      <!-- 150 -->
      <g transform="translate(383.868386 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-35"/>
       <use x="127.246094" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="xtick_8">
     <g id="line2d_8">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="449.166195" xlink:href="#m0a42397935" y="378"/>
      </g>
     </g>
     <g id="text_8">
      <!-- 175 -->
      <g transform="translate(434.85057 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-31"/>
       <use x="63.623047" xlink:href="#DejaVuSans-37"/>
       <use x="127.246094" xlink:href="#DejaVuSans-35"/>
      </g>
     </g>
    </g>
    <g id="xtick_9">
     <g id="line2d_9">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="500.148378" xlink:href="#m0a42397935" y="378"/>
      </g>
     </g>
     <g id="text_9">
      <!-- 200 -->
      <g transform="translate(485.832753 396.397656)scale(0.15 -0.15)">
       <use xlink:href="#DejaVuSans-32"/>
       <use x="63.623047" xlink:href="#DejaVuSans-30"/>
       <use x="127.246094" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="text_10">
     <!-- Iteration number, $k$ -->
     <g transform="translate(222.6 414.914844)scale(0.15 -0.15)">
      <defs>
       <path d="M 628 4666 
L 1259 4666 
L 1259 0 
L 628 0 
L 628 4666 
z
" id="DejaVuSans-49" transform="scale(0.015625)"/>
       <path d="M 1172 4494 
L 1172 3500 
L 2356 3500 
L 2356 3053 
L 1172 3053 
L 1172 1153 
Q 1172 725 1289 603 
Q 1406 481 1766 481 
L 2356 481 
L 2356 0 
L 1766 0 
Q 1100 0 847 248 
Q 594 497 594 1153 
L 594 3053 
L 172 3053 
L 172 3500 
L 594 3500 
L 594 4494 
L 1172 4494 
z
" id="DejaVuSans-74" transform="scale(0.015625)"/>
       <path d="M 3597 1894 
L 3597 1613 
L 953 1613 
Q 991 1019 1311 708 
Q 1631 397 2203 397 
Q 2534 397 2845 478 
Q 3156 559 3463 722 
L 3463 178 
Q 3153 47 2828 -22 
Q 2503 -91 2169 -91 
Q 1331 -91 842 396 
Q 353 884 353 1716 
Q 353 2575 817 3079 
Q 1281 3584 2069 3584 
Q 2775 3584 3186 3129 
Q 3597 2675 3597 1894 
z
M 3022 2063 
Q 3016 2534 2758 2815 
Q 2500 3097 2075 3097 
Q 1594 3097 1305 2825 
Q 1016 2553 972 2059 
L 3022 2063 
z
" id="DejaVuSans-65" transform="scale(0.015625)"/>
       <path d="M 2631 2963 
Q 2534 3019 2420 3045 
Q 2306 3072 2169 3072 
Q 1681 3072 1420 2755 
Q 1159 2438 1159 1844 
L 1159 0 
L 581 0 
L 581 3500 
L 1159 3500 
L 1159 2956 
Q 1341 3275 1631 3429 
Q 1922 3584 2338 3584 
Q 2397 3584 2469 3576 
Q 2541 3569 2628 3553 
L 2631 2963 
z
" id="DejaVuSans-72" transform="scale(0.015625)"/>
       <path d="M 2194 1759 
Q 1497 1759 1228 1600 
Q 959 1441 959 1056 
Q 959 750 1161 570 
Q 1363 391 1709 391 
Q 2188 391 2477 730 
Q 2766 1069 2766 1631 
L 2766 1759 
L 2194 1759 
z
M 3341 1997 
L 3341 0 
L 2766 0 
L 2766 531 
Q 2569 213 2275 61 
Q 1981 -91 1556 -91 
Q 1019 -91 701 211 
Q 384 513 384 1019 
Q 384 1609 779 1909 
Q 1175 2209 1959 2209 
L 2766 2209 
L 2766 2266 
Q 2766 2663 2505 2880 
Q 2244 3097 1772 3097 
Q 1472 3097 1187 3025 
Q 903 2953 641 2809 
L 641 3341 
Q 956 3463 1253 3523 
Q 1550 3584 1831 3584 
Q 2591 3584 2966 3190 
Q 3341 2797 3341 1997 
z
" id="DejaVuSans-61" transform="scale(0.015625)"/>
       <path d="M 603 3500 
L 1178 3500 
L 1178 0 
L 603 0 
L 603 3500 
z
M 603 4863 
L 1178 4863 
L 1178 4134 
L 603 4134 
L 603 4863 
z
" id="DejaVuSans-69" transform="scale(0.015625)"/>
       <path d="M 1959 3097 
Q 1497 3097 1228 2736 
Q 959 2375 959 1747 
Q 959 1119 1226 758 
Q 1494 397 1959 397 
Q 2419 397 2687 759 
Q 2956 1122 2956 1747 
Q 2956 2369 2687 2733 
Q 2419 3097 1959 3097 
z
M 1959 3584 
Q 2709 3584 3137 3096 
Q 3566 2609 3566 1747 
Q 3566 888 3137 398 
Q 2709 -91 1959 -91 
Q 1206 -91 779 398 
Q 353 888 353 1747 
Q 353 2609 779 3096 
Q 1206 3584 1959 3584 
z
" id="DejaVuSans-6f" transform="scale(0.015625)"/>
       <path d="M 3513 2113 
L 3513 0 
L 2938 0 
L 2938 2094 
Q 2938 2591 2744 2837 
Q 2550 3084 2163 3084 
Q 1697 3084 1428 2787 
Q 1159 2491 1159 1978 
L 1159 0 
L 581 0 
L 581 3500 
L 1159 3500 
L 1159 2956 
Q 1366 3272 1645 3428 
Q 1925 3584 2291 3584 
Q 2894 3584 3203 3211 
Q 3513 2838 3513 2113 
z
" id="DejaVuSans-6e" transform="scale(0.015625)"/>
       <path id="DejaVuSans-20" transform="scale(0.015625)"/>
       <path d="M 544 1381 
L 544 3500 
L 1119 3500 
L 1119 1403 
Q 1119 906 1312 657 
Q 1506 409 1894 409 
Q 2359 409 2629 706 
Q 2900 1003 2900 1516 
L 2900 3500 
L 3475 3500 
L 3475 0 
L 2900 0 
L 2900 538 
Q 2691 219 2414 64 
Q 2138 -91 1772 -91 
Q 1169 -91 856 284 
Q 544 659 544 1381 
z
M 1991 3584 
L 1991 3584 
z
" id="DejaVuSans-75" transform="scale(0.015625)"/>
       <path d="M 3328 2828 
Q 3544 3216 3844 3400 
Q 4144 3584 4550 3584 
Q 5097 3584 5394 3201 
Q 5691 2819 5691 2113 
L 5691 0 
L 5113 0 
L 5113 2094 
Q 5113 2597 4934 2840 
Q 4756 3084 4391 3084 
Q 3944 3084 3684 2787 
Q 3425 2491 3425 1978 
L 3425 0 
L 2847 0 
L 2847 2094 
Q 2847 2600 2669 2842 
Q 2491 3084 2119 3084 
Q 1678 3084 1418 2786 
Q 1159 2488 1159 1978 
L 1159 0 
L 581 0 
L 581 3500 
L 1159 3500 
L 1159 2956 
Q 1356 3278 1631 3431 
Q 1906 3584 2284 3584 
Q 2666 3584 2933 3390 
Q 3200 3197 3328 2828 
z
" id="DejaVuSans-6d" transform="scale(0.015625)"/>
       <path d="M 3116 1747 
Q 3116 2381 2855 2742 
Q 2594 3103 2138 3103 
Q 1681 3103 1420 2742 
Q 1159 2381 1159 1747 
Q 1159 1113 1420 752 
Q 1681 391 2138 391 
Q 2594 391 2855 752 
Q 3116 1113 3116 1747 
z
M 1159 2969 
Q 1341 3281 1617 3432 
Q 1894 3584 2278 3584 
Q 2916 3584 3314 3078 
Q 3713 2572 3713 1747 
Q 3713 922 3314 415 
Q 2916 -91 2278 -91 
Q 1894 -91 1617 61 
Q 1341 213 1159 525 
L 1159 0 
L 581 0 
L 581 4863 
L 1159 4863 
L 1159 2969 
z
" id="DejaVuSans-62" transform="scale(0.015625)"/>
       <path d="M 750 794 
L 1409 794 
L 1409 256 
L 897 -744 
L 494 -744 
L 750 256 
L 750 794 
z
" id="DejaVuSans-2c" transform="scale(0.015625)"/>
       <path d="M 1172 4863 
L 1747 4863 
L 1197 2028 
L 3169 3500 
L 3916 3500 
L 1716 1825 
L 3322 0 
L 2625 0 
L 1131 1709 
L 800 0 
L 225 0 
L 1172 4863 
z
" id="DejaVuSans-Oblique-6b" transform="scale(0.015625)"/>
      </defs>
      <use transform="translate(0 0.015625)" xlink:href="#DejaVuSans-49"/>
      <use transform="translate(29.492188 0.015625)" xlink:href="#DejaVuSans-74"/>
      <use transform="translate(68.701172 0.015625)" xlink:href="#DejaVuSans-65"/>
      <use transform="translate(130.224609 0.015625)" xlink:href="#DejaVuSans-72"/>
      <use transform="translate(171.337891 0.015625)" xlink:href="#DejaVuSans-61"/>
      <use transform="translate(232.617188 0.015625)" xlink:href="#DejaVuSans-74"/>
      <use transform="translate(271.826172 0.015625)" xlink:href="#DejaVuSans-69"/>
      <use transform="translate(299.609375 0.015625)" xlink:href="#DejaVuSans-6f"/>
      <use transform="translate(360.791016 0.015625)" xlink:href="#DejaVuSans-6e"/>
      <use transform="translate(424.169922 0.015625)" xlink:href="#DejaVuSans-20"/>
      <use transform="translate(455.957031 0.015625)" xlink:href="#DejaVuSans-6e"/>
      <use transform="translate(519.335938 0.015625)" xlink:href="#DejaVuSans-75"/>
      <use transform="translate(582.714844 0.015625)" xlink:href="#DejaVuSans-6d"/>
      <use transform="translate(680.126953 0.015625)" xlink:href="#DejaVuSans-62"/>
      <use transform="translate(743.603516 0.015625)" xlink:href="#DejaVuSans-65"/>
      <use transform="translate(805.126953 0.015625)" xlink:href="#DejaVuSans-72"/>
      <use transform="translate(846.240234 0.015625)" xlink:href="#DejaVuSans-2c"/>
      <use transform="translate(878.027344 0.015625)" xlink:href="#DejaVuSans-20"/>
      <use transform="translate(909.814453 0.015625)" xlink:href="#DejaVuSans-Oblique-6b"/>
     </g>
    </g>
   </g>
   <g id="matplotlib.axis_2">
    <g id="ytick_1">
     <g id="line2d_10">
      <defs>
       <path d="M 0 0 
L -3.5 0 
" id="ma13c6aa503" style="stroke:#000000;stroke-width:0.8;"/>
      </defs>
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#ma13c6aa503" y="345.324184"/>
      </g>
     </g>
     <g id="text_11">
      <!-- $\mathdefault{10^{-28}}$ -->
      <g transform="translate(23.15 351.023012)scale(0.15 -0.15)">
       <defs>
        <path d="M 678 2272 
L 4684 2272 
L 4684 1741 
L 678 1741 
L 678 2272 
z
" id="DejaVuSans-2212" transform="scale(0.015625)"/>
        <path d="M 2034 2216 
Q 1584 2216 1326 1975 
Q 1069 1734 1069 1313 
Q 1069 891 1326 650 
Q 1584 409 2034 409 
Q 2484 409 2743 651 
Q 3003 894 3003 1313 
Q 3003 1734 2745 1975 
Q 2488 2216 2034 2216 
z
M 1403 2484 
Q 997 2584 770 2862 
Q 544 3141 544 3541 
Q 544 4100 942 4425 
Q 1341 4750 2034 4750 
Q 2731 4750 3128 4425 
Q 3525 4100 3525 3541 
Q 3525 3141 3298 2862 
Q 3072 2584 2669 2484 
Q 3125 2378 3379 2068 
Q 3634 1759 3634 1313 
Q 3634 634 3220 271 
Q 2806 -91 2034 -91 
Q 1263 -91 848 271 
Q 434 634 434 1313 
Q 434 1759 690 2068 
Q 947 2378 1403 2484 
z
M 1172 3481 
Q 1172 3119 1398 2916 
Q 1625 2713 2034 2713 
Q 2441 2713 2670 2916 
Q 2900 3119 2900 3481 
Q 2900 3844 2670 4047 
Q 2441 4250 2034 4250 
Q 1625 4250 1398 4047 
Q 1172 3844 1172 3481 
z
" id="DejaVuSans-38" transform="scale(0.015625)"/>
       </defs>
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-38"/>
      </g>
     </g>
    </g>
    <g id="ytick_2">
     <g id="line2d_11">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#ma13c6aa503" y="307.177353"/>
      </g>
     </g>
     <g id="text_12">
      <!-- $\mathdefault{10^{-24}}$ -->
      <g transform="translate(23.15 312.876182)scale(0.15 -0.15)">
       <defs>
        <path d="M 2419 4116 
L 825 1625 
L 2419 1625 
L 2419 4116 
z
M 2253 4666 
L 3047 4666 
L 3047 1625 
L 3713 1625 
L 3713 1100 
L 3047 1100 
L 3047 0 
L 2419 0 
L 2419 1100 
L 313 1100 
L 313 1709 
L 2253 4666 
z
" id="DejaVuSans-34" transform="scale(0.015625)"/>
       </defs>
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-34"/>
      </g>
     </g>
    </g>
    <g id="ytick_3">
     <g id="line2d_12">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#ma13c6aa503" y="269.030523"/>
      </g>
     </g>
     <g id="text_13">
      <!-- $\mathdefault{10^{-20}}$ -->
      <g transform="translate(23.15 274.729351)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="ytick_4">
     <g id="line2d_13">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#ma13c6aa503" y="230.883692"/>
      </g>
     </g>
     <g id="text_14">
      <!-- $\mathdefault{10^{-16}}$ -->
      <g transform="translate(23.15 236.582521)scale(0.15 -0.15)">
       <defs>
        <path d="M 2113 2584 
Q 1688 2584 1439 2293 
Q 1191 2003 1191 1497 
Q 1191 994 1439 701 
Q 1688 409 2113 409 
Q 2538 409 2786 701 
Q 3034 994 3034 1497 
Q 3034 2003 2786 2293 
Q 2538 2584 2113 2584 
z
M 3366 4563 
L 3366 3988 
Q 3128 4100 2886 4159 
Q 2644 4219 2406 4219 
Q 1781 4219 1451 3797 
Q 1122 3375 1075 2522 
Q 1259 2794 1537 2939 
Q 1816 3084 2150 3084 
Q 2853 3084 3261 2657 
Q 3669 2231 3669 1497 
Q 3669 778 3244 343 
Q 2819 -91 2113 -91 
Q 1303 -91 875 529 
Q 447 1150 447 2328 
Q 447 3434 972 4092 
Q 1497 4750 2381 4750 
Q 2619 4750 2861 4703 
Q 3103 4656 3366 4563 
z
" id="DejaVuSans-36" transform="scale(0.015625)"/>
       </defs>
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-36"/>
      </g>
     </g>
    </g>
    <g id="ytick_5">
     <g id="line2d_14">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#ma13c6aa503" y="192.736862"/>
      </g>
     </g>
     <g id="text_15">
      <!-- $\mathdefault{10^{-12}}$ -->
      <g transform="translate(23.15 198.43569)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(231.391602 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
      </g>
     </g>
    </g>
    <g id="ytick_6">
     <g id="line2d_15">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#ma13c6aa503" y="154.590031"/>
      </g>
     </g>
     <g id="text_16">
      <!-- $\mathdefault{10^{-8}}$ -->
      <g transform="translate(29.75 160.28886)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 39.046875)scale(0.7)" xlink:href="#DejaVuSans-38"/>
      </g>
     </g>
    </g>
    <g id="ytick_7">
     <g id="line2d_16">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#ma13c6aa503" y="116.443201"/>
      </g>
     </g>
     <g id="text_17">
      <!-- $\mathdefault{10^{-4}}$ -->
      <g transform="translate(29.75 122.142029)scale(0.15 -0.15)">
       <use transform="translate(0 0.684375)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.684375)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 38.965625)scale(0.7)" xlink:href="#DejaVuSans-2212"/>
       <use transform="translate(186.855469 38.965625)scale(0.7)" xlink:href="#DejaVuSans-34"/>
      </g>
     </g>
    </g>
    <g id="ytick_8">
     <g id="line2d_17">
      <g>
       <use style="stroke:#000000;stroke-width:0.8;" x="72" xlink:href="#ma13c6aa503" y="78.29637"/>
      </g>
     </g>
     <g id="text_18">
      <!-- $\mathdefault{10^{0}}$ -->
      <g transform="translate(38.6 83.995199)scale(0.15 -0.15)">
       <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-31"/>
       <use transform="translate(63.623047 0.765625)" xlink:href="#DejaVuSans-30"/>
       <use transform="translate(128.203125 39.046875)scale(0.7)" xlink:href="#DejaVuSans-30"/>
      </g>
     </g>
    </g>
    <g id="text_19">
     <!-- $||c_k-c*||^2$ -->
     <g transform="translate(15.55 256.02)rotate(-90)scale(0.15 -0.15)">
      <defs>
       <path d="M 1344 4891 
L 1344 -1509 
L 813 -1509 
L 813 4891 
L 1344 4891 
z
" id="DejaVuSans-7c" transform="scale(0.015625)"/>
       <path d="M 3431 3366 
L 3316 2797 
Q 3109 2947 2876 3022 
Q 2644 3097 2394 3097 
Q 2119 3097 1870 3000 
Q 1622 2903 1453 2725 
Q 1184 2453 1037 2087 
Q 891 1722 891 1331 
Q 891 859 1127 628 
Q 1363 397 1844 397 
Q 2081 397 2348 469 
Q 2616 541 2906 684 
L 2797 116 
Q 2547 13 2283 -39 
Q 2019 -91 1741 -91 
Q 1044 -91 669 257 
Q 294 606 294 1253 
Q 294 1797 489 2255 
Q 684 2713 1069 3078 
Q 1331 3328 1684 3456 
Q 2038 3584 2456 3584 
Q 2700 3584 2940 3529 
Q 3181 3475 3431 3366 
z
" id="DejaVuSans-Oblique-63" transform="scale(0.015625)"/>
       <path d="M 3009 3897 
L 1888 3291 
L 3009 2681 
L 2828 2375 
L 1778 3009 
L 1778 1831 
L 1422 1831 
L 1422 3009 
L 372 2375 
L 191 2681 
L 1313 3291 
L 191 3897 
L 372 4206 
L 1422 3572 
L 1422 4750 
L 1778 4750 
L 1778 3572 
L 2828 4206 
L 3009 3897 
z
" id="DejaVuSans-2a" transform="scale(0.015625)"/>
      </defs>
      <use transform="translate(0 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(33.691406 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(67.382812 0.765625)" xlink:href="#DejaVuSans-Oblique-63"/>
      <use transform="translate(122.363281 -15.640625)scale(0.7)" xlink:href="#DejaVuSans-Oblique-6b"/>
      <use transform="translate(185.117188 0.765625)" xlink:href="#DejaVuSans-2212"/>
      <use transform="translate(288.388672 0.765625)" xlink:href="#DejaVuSans-Oblique-63"/>
      <use transform="translate(362.851562 0.765625)" xlink:href="#DejaVuSans-2a"/>
      <use transform="translate(432.333984 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(466.025391 0.765625)" xlink:href="#DejaVuSans-7c"/>
      <use transform="translate(500.673828 39.046875)scale(0.7)" xlink:href="#DejaVuSans-32"/>
     </g>
    </g>
   </g>
   <g id="line2d_18">
    <path clip-path="url(#pcfdc21f5b5)" d="M 92.290909 66.673767 
L 98.408771 66.856056 
L 100.448058 66.874323 
L 102.487346 67.159954 
L 108.605208 67.238048 
L 112.683783 67.59117 
L 120.840932 67.681127 
L 141.233805 67.90219 
L 143.273093 67.919221 
L 145.31238 68.086932 
L 149.390955 68.202911 
L 151.430242 68.407996 
L 157.548104 68.557377 
L 161.626679 68.818865 
L 167.744541 68.934778 
L 210.569575 69.809414 
L 212.608862 70.201396 
L 216.687437 70.307944 
L 222.805299 70.42132 
L 230.962449 70.655299 
L 237.080311 71.06014 
L 239.119598 71.213242 
L 249.316035 71.287898 
L 253.394609 71.378381 
L 271.748196 71.666475 
L 273.787483 71.871261 
L 275.82677 71.889201 
L 277.866058 72.166534 
L 298.258931 72.352031 
L 300.298218 72.682179 
L 302.337506 72.832328 
L 339.044678 73.139468 
L 343.123253 73.234105 
L 363.516126 73.368947 
L 365.555413 73.554312 
L 367.594701 73.603354 
L 369.633988 73.809105 
L 373.712563 73.870352 
L 375.75185 74.043125 
L 385.948287 74.106532 
L 390.026862 74.319961 
L 392.066149 74.343099 
L 394.105436 74.872772 
L 422.655459 75.087842 
L 424.694746 75.39659 
L 428.773321 75.492728 
L 487.912654 76.024648 
L 489.951942 76.156519 
L 498.109091 76.206782 
L 498.109091 76.206782 
" style="fill:none;stroke:#0000ff;stroke-linecap:square;stroke-width:3;"/>
   </g>
   <g id="line2d_19">
    <path clip-path="url(#pcfdc21f5b5)" d="M 92.290909 67.939464 
L 94.330196 71.198172 
L 96.369484 73.269243 
L 98.408771 74.422961 
L 100.448058 74.509971 
L 102.487346 75.05036 
L 104.526633 77.805047 
L 106.565921 79.434349 
L 108.605208 81.970325 
L 110.644495 83.989491 
L 112.683783 85.307898 
L 114.72307 86.272377 
L 116.762357 86.381552 
L 118.801645 89.712643 
L 120.840932 90.486881 
L 122.880219 93.624844 
L 124.919507 95.56306 
L 126.958794 96.596866 
L 128.998081 97.032147 
L 131.037369 97.193652 
L 133.076656 101.042841 
L 135.115943 101.800708 
L 137.155231 101.805582 
L 139.194518 103.557396 
L 141.233805 103.93164 
L 143.273093 104.462275 
L 145.31238 104.806042 
L 149.390955 109.411676 
L 153.469529 114.124956 
L 155.508817 114.124956 
L 157.548104 116.564851 
L 159.587392 117.637988 
L 163.665966 123.210993 
L 167.744541 128.435159 
L 169.783828 130.260098 
L 171.823116 132.459314 
L 173.862403 134.480894 
L 175.90169 135.609581 
L 177.940978 138.969826 
L 179.980265 140.551559 
L 182.019552 143.666076 
L 184.05884 145.197131 
L 186.098127 147.876361 
L 188.137414 148.181337 
L 190.176702 148.18157 
L 192.215989 151.403303 
L 194.255276 151.834453 
L 196.294564 154.214508 
L 198.333851 154.639262 
L 200.373138 157.40462 
L 202.412426 157.43777 
L 204.451713 158.982036 
L 206.491 162.133642 
L 212.608862 169.25536 
L 214.64815 170.542019 
L 216.687437 173.44498 
L 218.726725 176.839429 
L 220.766012 178.758457 
L 222.805299 181.067635 
L 224.844587 183.563257 
L 226.883874 184.289273 
L 228.923161 186.892106 
L 230.962449 188.667727 
L 233.001736 191.748006 
L 235.041023 192.4409 
L 237.080311 192.555022 
L 239.119598 195.263714 
L 241.158885 198.562008 
L 243.198173 200.240569 
L 245.23746 202.116808 
L 247.276747 204.9179 
L 249.316035 208.036451 
L 251.355322 210.506556 
L 253.394609 212.582403 
L 255.433897 214.335231 
L 257.473184 214.427009 
L 259.512471 216.355467 
L 261.551759 217.305177 
L 265.630333 219.727251 
L 267.669621 220.409315 
L 269.708908 220.474002 
L 273.787483 226.246082 
L 275.82677 229.607267 
L 277.866058 232.408022 
L 279.905345 233.714914 
L 281.944632 234.340395 
L 283.98392 237.424146 
L 286.023207 239.800484 
L 288.062494 241.987008 
L 290.101782 243.964045 
L 292.141069 245.11387 
L 296.219644 250.928187 
L 300.298218 255.131318 
L 302.337506 257.379311 
L 304.376793 259.805606 
L 306.41608 263.311269 
L 308.455368 263.414285 
L 310.494655 264.078047 
L 312.533942 267.406511 
L 314.57323 270.010237 
L 316.612517 271.732019 
L 320.691092 277.714794 
L 322.730379 279.780076 
L 324.769667 282.068311 
L 326.808954 283.639125 
L 328.848241 285.496859 
L 330.887529 287.68617 
L 332.926816 288.799992 
L 339.044678 297.376858 
L 341.083965 299.201692 
L 343.123253 300.197076 
L 345.16254 302.660976 
L 347.201827 305.735242 
L 349.241115 308.150901 
L 351.280402 311.424817 
L 353.319689 311.433014 
L 355.358977 313.250437 
L 357.398264 313.999916 
L 359.437551 315.480088 
L 361.476839 318.390058 
L 363.516126 320.590768 
L 365.555413 323.779919 
L 367.594701 325.630193 
L 369.633988 325.885277 
L 371.673275 328.771442 
L 373.712563 329.334464 
L 375.75185 329.502116 
L 377.791138 331.631455 
L 379.830425 331.837663 
L 381.869712 332.987861 
L 383.909 336.171134 
L 385.948287 336.319951 
L 387.987574 336.922411 
L 390.026862 337.064064 
L 392.066149 337.788375 
L 394.105436 338.04775 
L 396.144724 339.92255 
L 398.184011 340.215888 
L 400.223298 342.921994 
L 402.262586 346.601466 
L 406.34116 351.130146 
L 408.380448 352.214509 
L 410.419735 352.493144 
L 412.459022 354.697214 
L 414.49831 357.166167 
L 416.537597 357.201949 
L 418.576884 357.597598 
L 420.616172 358.123906 
L 422.655459 359.905508 
L 424.694746 361.358182 
L 426.734034 362.288516 
L 428.773321 362.916754 
L 432.851896 362.988786 
L 434.891183 363.174545 
L 438.969758 363.062093 
L 441.009045 362.707883 
L 443.048333 362.674072 
L 445.08762 362.31931 
L 447.126907 362.31931 
L 449.166195 361.992552 
L 455.284057 361.407489 
L 459.362631 361.333747 
L 463.441206 361.097012 
L 498.109091 360.765496 
L 498.109091 360.765496 
" style="fill:none;stroke:#008000;stroke-dasharray:11.1,4.8;stroke-dashoffset:0;stroke-width:3;"/>
   </g>
   <g id="line2d_20">
    <path clip-path="url(#pcfdc21f5b5)" d="M 92.290909 66.665455 
L 98.408771 67.360562 
L 104.526633 67.9442 
L 114.72307 69.221465 
L 116.762357 69.334788 
L 118.801645 69.614083 
L 122.880219 69.857002 
L 124.919507 70.224322 
L 128.998081 70.402271 
L 135.115943 70.799853 
L 139.194518 71.403655 
L 141.233805 71.936805 
L 147.351667 72.400987 
L 151.430242 73.173393 
L 157.548104 73.355906 
L 159.587392 73.802543 
L 163.665966 73.873673 
L 165.705254 74.06928 
L 167.744541 74.151312 
L 169.783828 74.365827 
L 175.90169 74.493025 
L 177.940978 74.951026 
L 179.980265 74.968731 
L 182.019552 75.564107 
L 184.05884 75.615019 
L 186.098127 76.176545 
L 192.215989 76.328281 
L 194.255276 77.173444 
L 196.294564 77.242869 
L 198.333851 77.905707 
L 202.412426 78.047551 
L 204.451713 79.044723 
L 206.491 79.692151 
L 212.608862 79.798136 
L 216.687437 80.269875 
L 228.923161 80.720224 
L 230.962449 82.805995 
L 235.041023 83.028393 
L 239.119598 83.206793 
L 241.158885 83.268863 
L 243.198173 84.674919 
L 245.23746 84.802041 
L 251.355322 84.910209 
L 253.394609 85.11631 
L 263.591046 85.40997 
L 265.630333 85.764363 
L 267.669621 85.919081 
L 275.82677 86.034257 
L 283.98392 86.252127 
L 286.023207 86.453402 
L 288.062494 86.787671 
L 292.141069 86.865966 
L 294.180356 87.266903 
L 300.298218 87.365944 
L 302.337506 92.588948 
L 304.376793 93.353079 
L 308.455368 93.638088 
L 310.494655 93.698351 
L 312.533942 93.892611 
L 314.57323 95.214501 
L 316.612517 95.480852 
L 320.691092 95.642139 
L 322.730379 96.151332 
L 324.769667 96.205121 
L 326.808954 96.574804 
L 330.887529 96.888939 
L 332.926816 97.295466 
L 337.005391 97.468904 
L 339.044678 98.334501 
L 343.123253 98.46838 
L 345.16254 98.962809 
L 349.241115 99.141951 
L 353.319689 99.205596 
L 355.358977 99.891695 
L 357.398264 100.201094 
L 359.437551 100.296645 
L 361.476839 100.513648 
L 363.516126 101.520238 
L 367.594701 101.636355 
L 373.712563 101.754473 
L 375.75185 101.891596 
L 385.948287 102.034924 
L 387.987574 104.19238 
L 394.105436 104.314888 
L 396.144724 104.494319 
L 400.223298 104.589686 
L 408.380448 105.016634 
L 410.419735 107.739611 
L 412.459022 108.894195 
L 418.576884 109.17614 
L 420.616172 109.501518 
L 426.734034 109.857996 
L 428.773321 109.879005 
L 430.812608 110.309763 
L 436.930471 110.721684 
L 438.969758 110.804637 
L 441.009045 111.232312 
L 445.08762 111.303445 
L 449.166195 111.638448 
L 455.284057 111.844456 
L 457.323344 112.013621 
L 469.559068 112.282069 
L 475.67693 112.555372 
L 498.109091 112.980724 
L 498.109091 112.980724 
" style="fill:none;stroke:#ff0000;stroke-dasharray:3,4.95;stroke-dashoffset:0;stroke-width:3;"/>
   </g>
   <g id="line2d_21">
    <path clip-path="url(#pcfdc21f5b5)" d="M 92.290909 67.285996 
L 98.408771 68.507653 
L 100.448058 68.599382 
L 102.487346 69.206899 
L 104.526633 69.466695 
L 106.565921 69.511365 
L 108.605208 69.842438 
L 110.644495 70.308998 
L 112.683783 71.039888 
L 120.840932 72.465921 
L 126.958794 73.367651 
L 131.037369 73.590582 
L 133.076656 73.613939 
L 135.115943 73.827503 
L 139.194518 74.551036 
L 147.351667 75.189301 
L 149.390955 75.539216 
L 151.430242 76.048341 
L 155.508817 76.239989 
L 157.548104 76.597082 
L 165.705254 77.464145 
L 167.744541 77.780261 
L 169.783828 78.712588 
L 171.823116 78.85328 
L 173.862403 79.137153 
L 175.90169 79.278099 
L 177.940978 79.835604 
L 179.980265 80.219274 
L 182.019552 80.749231 
L 184.05884 81.047276 
L 186.098127 81.588714 
L 190.176702 81.682391 
L 194.255276 82.303698 
L 196.294564 83.208249 
L 202.412426 84.340651 
L 204.451713 84.583387 
L 206.491 84.99539 
L 208.530288 85.53113 
L 210.569575 85.947564 
L 214.64815 86.551399 
L 220.766012 86.787413 
L 224.844587 87.071867 
L 226.883874 88.536723 
L 230.962449 89.236272 
L 233.001736 89.760764 
L 235.041023 89.986006 
L 237.080311 90.09302 
L 241.158885 90.547164 
L 245.23746 90.785944 
L 247.276747 91.322075 
L 249.316035 91.657202 
L 251.355322 91.788508 
L 253.394609 92.521755 
L 257.473184 92.998543 
L 259.512471 93.275861 
L 261.551759 93.981668 
L 263.591046 94.180313 
L 269.708908 94.497954 
L 271.748196 94.644271 
L 273.787483 95.041456 
L 281.944632 95.489167 
L 283.98392 95.770338 
L 286.023207 95.874551 
L 288.062494 96.842517 
L 290.101782 97.121081 
L 294.180356 97.273524 
L 296.219644 97.72919 
L 300.298218 98.052345 
L 302.337506 98.092335 
L 306.41608 98.805819 
L 308.455368 98.96247 
L 310.494655 99.382237 
L 312.533942 99.637459 
L 314.57323 99.732082 
L 320.691092 100.415289 
L 322.730379 100.574555 
L 324.769667 100.96957 
L 326.808954 101.098488 
L 328.848241 101.757062 
L 330.887529 102.562904 
L 332.926816 102.866171 
L 339.044678 103.206531 
L 341.083965 103.46546 
L 343.123253 103.602041 
L 345.16254 104.046431 
L 347.201827 104.290064 
L 351.280402 104.486989 
L 353.319689 105.310977 
L 359.437551 106.117578 
L 361.476839 106.626967 
L 365.555413 107.059626 
L 367.594701 107.142722 
L 369.633988 107.737945 
L 371.673275 108.103331 
L 377.791138 108.550929 
L 379.830425 109.794952 
L 381.869712 109.811478 
L 385.948287 110.48065 
L 387.987574 111.059021 
L 390.026862 111.102794 
L 392.066149 111.261241 
L 394.105436 111.603713 
L 396.144724 111.752634 
L 398.184011 112.344931 
L 400.223298 112.661905 
L 402.262586 112.680423 
L 406.34116 113.050738 
L 408.380448 113.147637 
L 410.419735 113.536285 
L 420.616172 113.890141 
L 426.734034 114.666162 
L 428.773321 114.757421 
L 430.812608 115.008634 
L 432.851896 115.066469 
L 436.930471 115.356562 
L 438.969758 115.391668 
L 441.009045 117.775378 
L 443.048333 118.205657 
L 455.284057 118.963017 
L 457.323344 119.325343 
L 459.362631 119.962234 
L 461.401919 120.306676 
L 463.441206 120.407154 
L 465.480493 120.622878 
L 469.559068 120.693068 
L 471.598355 121.087502 
L 475.67693 121.605027 
L 479.755505 121.748803 
L 485.873367 122.008536 
L 489.951942 122.1421 
L 491.991229 122.159138 
L 494.030516 122.416034 
L 496.069804 122.416034 
L 498.109091 122.533153 
L 498.109091 122.533153 
" style="fill:none;stroke:#1f77b4;stroke-dasharray:19.2,4.8,3,4.8;stroke-dashoffset:0;stroke-width:3;"/>
    <defs>
     <path d="M 0 -3 
L -2.85317 -0.927051 
L -1.763356 2.427051 
L 1.763356 2.427051 
L 2.85317 -0.927051 
z
" id="m6ce50a83c0" style="stroke:#1f77b4;stroke-linejoin:miter;"/>
    </defs>
    <g clip-path="url(#pcfdc21f5b5)">
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="92.290909" xlink:href="#m6ce50a83c0" y="67.285996"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="94.330196" xlink:href="#m6ce50a83c0" y="67.710494"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="96.369484" xlink:href="#m6ce50a83c0" y="68.032013"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="98.408771" xlink:href="#m6ce50a83c0" y="68.507653"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="100.448058" xlink:href="#m6ce50a83c0" y="68.599382"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="102.487346" xlink:href="#m6ce50a83c0" y="69.206899"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="104.526633" xlink:href="#m6ce50a83c0" y="69.466695"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="106.565921" xlink:href="#m6ce50a83c0" y="69.511365"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="108.605208" xlink:href="#m6ce50a83c0" y="69.842438"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="110.644495" xlink:href="#m6ce50a83c0" y="70.308998"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="112.683783" xlink:href="#m6ce50a83c0" y="71.039888"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="114.72307" xlink:href="#m6ce50a83c0" y="71.414786"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="116.762357" xlink:href="#m6ce50a83c0" y="71.885949"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="118.801645" xlink:href="#m6ce50a83c0" y="72.196463"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="120.840932" xlink:href="#m6ce50a83c0" y="72.465921"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="122.880219" xlink:href="#m6ce50a83c0" y="72.781239"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="124.919507" xlink:href="#m6ce50a83c0" y="73.201907"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="126.958794" xlink:href="#m6ce50a83c0" y="73.367651"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="128.998081" xlink:href="#m6ce50a83c0" y="73.520441"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="131.037369" xlink:href="#m6ce50a83c0" y="73.590582"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="133.076656" xlink:href="#m6ce50a83c0" y="73.613939"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="135.115943" xlink:href="#m6ce50a83c0" y="73.827503"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="137.155231" xlink:href="#m6ce50a83c0" y="74.205676"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="139.194518" xlink:href="#m6ce50a83c0" y="74.551036"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="141.233805" xlink:href="#m6ce50a83c0" y="74.68628"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="143.273093" xlink:href="#m6ce50a83c0" y="74.931088"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="145.31238" xlink:href="#m6ce50a83c0" y="74.98432"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="147.351667" xlink:href="#m6ce50a83c0" y="75.189301"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="149.390955" xlink:href="#m6ce50a83c0" y="75.539216"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="151.430242" xlink:href="#m6ce50a83c0" y="76.048341"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="153.469529" xlink:href="#m6ce50a83c0" y="76.185846"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="155.508817" xlink:href="#m6ce50a83c0" y="76.239989"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="157.548104" xlink:href="#m6ce50a83c0" y="76.597082"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="159.587392" xlink:href="#m6ce50a83c0" y="76.797842"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="161.626679" xlink:href="#m6ce50a83c0" y="76.910017"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="163.665966" xlink:href="#m6ce50a83c0" y="77.091529"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="165.705254" xlink:href="#m6ce50a83c0" y="77.464145"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="167.744541" xlink:href="#m6ce50a83c0" y="77.780261"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="169.783828" xlink:href="#m6ce50a83c0" y="78.712588"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="171.823116" xlink:href="#m6ce50a83c0" y="78.85328"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="173.862403" xlink:href="#m6ce50a83c0" y="79.137153"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="175.90169" xlink:href="#m6ce50a83c0" y="79.278099"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="177.940978" xlink:href="#m6ce50a83c0" y="79.835604"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="179.980265" xlink:href="#m6ce50a83c0" y="80.219274"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="182.019552" xlink:href="#m6ce50a83c0" y="80.749231"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="184.05884" xlink:href="#m6ce50a83c0" y="81.047276"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="186.098127" xlink:href="#m6ce50a83c0" y="81.588714"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="188.137414" xlink:href="#m6ce50a83c0" y="81.682391"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="190.176702" xlink:href="#m6ce50a83c0" y="81.682391"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="192.215989" xlink:href="#m6ce50a83c0" y="82.042549"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="194.255276" xlink:href="#m6ce50a83c0" y="82.303698"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="196.294564" xlink:href="#m6ce50a83c0" y="83.208249"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="198.333851" xlink:href="#m6ce50a83c0" y="83.60866"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="200.373138" xlink:href="#m6ce50a83c0" y="84.064926"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="202.412426" xlink:href="#m6ce50a83c0" y="84.340651"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="204.451713" xlink:href="#m6ce50a83c0" y="84.583387"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="206.491" xlink:href="#m6ce50a83c0" y="84.99539"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="208.530288" xlink:href="#m6ce50a83c0" y="85.53113"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="210.569575" xlink:href="#m6ce50a83c0" y="85.947564"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="212.608862" xlink:href="#m6ce50a83c0" y="86.246286"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="214.64815" xlink:href="#m6ce50a83c0" y="86.551399"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="216.687437" xlink:href="#m6ce50a83c0" y="86.625659"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="218.726725" xlink:href="#m6ce50a83c0" y="86.6325"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="220.766012" xlink:href="#m6ce50a83c0" y="86.787413"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="222.805299" xlink:href="#m6ce50a83c0" y="86.97627"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="224.844587" xlink:href="#m6ce50a83c0" y="87.071867"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="226.883874" xlink:href="#m6ce50a83c0" y="88.536723"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="228.923161" xlink:href="#m6ce50a83c0" y="88.832174"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="230.962449" xlink:href="#m6ce50a83c0" y="89.236272"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="233.001736" xlink:href="#m6ce50a83c0" y="89.760764"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="235.041023" xlink:href="#m6ce50a83c0" y="89.986006"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="237.080311" xlink:href="#m6ce50a83c0" y="90.09302"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="239.119598" xlink:href="#m6ce50a83c0" y="90.327084"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="241.158885" xlink:href="#m6ce50a83c0" y="90.547164"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="243.198173" xlink:href="#m6ce50a83c0" y="90.636621"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="245.23746" xlink:href="#m6ce50a83c0" y="90.785944"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="247.276747" xlink:href="#m6ce50a83c0" y="91.322075"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="249.316035" xlink:href="#m6ce50a83c0" y="91.657202"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="251.355322" xlink:href="#m6ce50a83c0" y="91.788508"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="253.394609" xlink:href="#m6ce50a83c0" y="92.521755"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="255.433897" xlink:href="#m6ce50a83c0" y="92.725865"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="257.473184" xlink:href="#m6ce50a83c0" y="92.998543"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="259.512471" xlink:href="#m6ce50a83c0" y="93.275861"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="261.551759" xlink:href="#m6ce50a83c0" y="93.981668"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="263.591046" xlink:href="#m6ce50a83c0" y="94.180313"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="265.630333" xlink:href="#m6ce50a83c0" y="94.261721"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="267.669621" xlink:href="#m6ce50a83c0" y="94.288096"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="269.708908" xlink:href="#m6ce50a83c0" y="94.497954"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="271.748196" xlink:href="#m6ce50a83c0" y="94.644271"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="273.787483" xlink:href="#m6ce50a83c0" y="95.041456"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="275.82677" xlink:href="#m6ce50a83c0" y="95.149508"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="277.866058" xlink:href="#m6ce50a83c0" y="95.179451"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="279.905345" xlink:href="#m6ce50a83c0" y="95.398724"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="281.944632" xlink:href="#m6ce50a83c0" y="95.489167"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="283.98392" xlink:href="#m6ce50a83c0" y="95.770338"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="286.023207" xlink:href="#m6ce50a83c0" y="95.874551"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="288.062494" xlink:href="#m6ce50a83c0" y="96.842517"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="290.101782" xlink:href="#m6ce50a83c0" y="97.121081"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="292.141069" xlink:href="#m6ce50a83c0" y="97.146833"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="294.180356" xlink:href="#m6ce50a83c0" y="97.273524"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="296.219644" xlink:href="#m6ce50a83c0" y="97.72919"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="298.258931" xlink:href="#m6ce50a83c0" y="97.927405"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="300.298218" xlink:href="#m6ce50a83c0" y="98.052345"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="302.337506" xlink:href="#m6ce50a83c0" y="98.092335"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="304.376793" xlink:href="#m6ce50a83c0" y="98.421915"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="306.41608" xlink:href="#m6ce50a83c0" y="98.805819"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="308.455368" xlink:href="#m6ce50a83c0" y="98.96247"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="310.494655" xlink:href="#m6ce50a83c0" y="99.382237"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="312.533942" xlink:href="#m6ce50a83c0" y="99.637459"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="314.57323" xlink:href="#m6ce50a83c0" y="99.732082"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="316.612517" xlink:href="#m6ce50a83c0" y="99.990429"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="318.651804" xlink:href="#m6ce50a83c0" y="100.211788"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="320.691092" xlink:href="#m6ce50a83c0" y="100.415289"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="322.730379" xlink:href="#m6ce50a83c0" y="100.574555"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="324.769667" xlink:href="#m6ce50a83c0" y="100.96957"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="326.808954" xlink:href="#m6ce50a83c0" y="101.098488"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="328.848241" xlink:href="#m6ce50a83c0" y="101.757062"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="330.887529" xlink:href="#m6ce50a83c0" y="102.562904"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="332.926816" xlink:href="#m6ce50a83c0" y="102.866171"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="334.966103" xlink:href="#m6ce50a83c0" y="102.980187"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="337.005391" xlink:href="#m6ce50a83c0" y="103.019932"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="339.044678" xlink:href="#m6ce50a83c0" y="103.206531"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="341.083965" xlink:href="#m6ce50a83c0" y="103.46546"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="343.123253" xlink:href="#m6ce50a83c0" y="103.602041"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="345.16254" xlink:href="#m6ce50a83c0" y="104.046431"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="347.201827" xlink:href="#m6ce50a83c0" y="104.290064"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="349.241115" xlink:href="#m6ce50a83c0" y="104.404155"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="351.280402" xlink:href="#m6ce50a83c0" y="104.486989"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="353.319689" xlink:href="#m6ce50a83c0" y="105.310977"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="355.358977" xlink:href="#m6ce50a83c0" y="105.583284"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="357.398264" xlink:href="#m6ce50a83c0" y="105.746551"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="359.437551" xlink:href="#m6ce50a83c0" y="106.117578"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="361.476839" xlink:href="#m6ce50a83c0" y="106.626967"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="363.516126" xlink:href="#m6ce50a83c0" y="106.841747"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="365.555413" xlink:href="#m6ce50a83c0" y="107.059626"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="367.594701" xlink:href="#m6ce50a83c0" y="107.142722"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="369.633988" xlink:href="#m6ce50a83c0" y="107.737945"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="371.673275" xlink:href="#m6ce50a83c0" y="108.103331"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="373.712563" xlink:href="#m6ce50a83c0" y="108.224893"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="375.75185" xlink:href="#m6ce50a83c0" y="108.312122"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="377.791138" xlink:href="#m6ce50a83c0" y="108.550929"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="379.830425" xlink:href="#m6ce50a83c0" y="109.794952"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="381.869712" xlink:href="#m6ce50a83c0" y="109.811478"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="383.909" xlink:href="#m6ce50a83c0" y="110.108112"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="385.948287" xlink:href="#m6ce50a83c0" y="110.48065"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="387.987574" xlink:href="#m6ce50a83c0" y="111.059021"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="390.026862" xlink:href="#m6ce50a83c0" y="111.102794"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="392.066149" xlink:href="#m6ce50a83c0" y="111.261241"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="394.105436" xlink:href="#m6ce50a83c0" y="111.603713"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="396.144724" xlink:href="#m6ce50a83c0" y="111.752634"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="398.184011" xlink:href="#m6ce50a83c0" y="112.344931"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="400.223298" xlink:href="#m6ce50a83c0" y="112.661905"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="402.262586" xlink:href="#m6ce50a83c0" y="112.680423"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="404.301873" xlink:href="#m6ce50a83c0" y="112.881927"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="406.34116" xlink:href="#m6ce50a83c0" y="113.050738"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="408.380448" xlink:href="#m6ce50a83c0" y="113.147637"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="410.419735" xlink:href="#m6ce50a83c0" y="113.536285"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="412.459022" xlink:href="#m6ce50a83c0" y="113.585933"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="414.49831" xlink:href="#m6ce50a83c0" y="113.651616"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="416.537597" xlink:href="#m6ce50a83c0" y="113.784028"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="418.576884" xlink:href="#m6ce50a83c0" y="113.799379"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="420.616172" xlink:href="#m6ce50a83c0" y="113.890141"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="422.655459" xlink:href="#m6ce50a83c0" y="114.138426"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="424.694746" xlink:href="#m6ce50a83c0" y="114.412644"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="426.734034" xlink:href="#m6ce50a83c0" y="114.666162"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="428.773321" xlink:href="#m6ce50a83c0" y="114.757421"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="430.812608" xlink:href="#m6ce50a83c0" y="115.008634"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="432.851896" xlink:href="#m6ce50a83c0" y="115.066469"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="434.891183" xlink:href="#m6ce50a83c0" y="115.244586"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="436.930471" xlink:href="#m6ce50a83c0" y="115.356562"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="438.969758" xlink:href="#m6ce50a83c0" y="115.391668"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="441.009045" xlink:href="#m6ce50a83c0" y="117.775378"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="443.048333" xlink:href="#m6ce50a83c0" y="118.205657"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="445.08762" xlink:href="#m6ce50a83c0" y="118.319931"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="447.126907" xlink:href="#m6ce50a83c0" y="118.391374"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="449.166195" xlink:href="#m6ce50a83c0" y="118.476831"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="451.205482" xlink:href="#m6ce50a83c0" y="118.690093"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="453.244769" xlink:href="#m6ce50a83c0" y="118.839998"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="455.284057" xlink:href="#m6ce50a83c0" y="118.963017"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="457.323344" xlink:href="#m6ce50a83c0" y="119.325343"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="459.362631" xlink:href="#m6ce50a83c0" y="119.962234"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="461.401919" xlink:href="#m6ce50a83c0" y="120.306676"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="463.441206" xlink:href="#m6ce50a83c0" y="120.407154"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="465.480493" xlink:href="#m6ce50a83c0" y="120.622878"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="467.519781" xlink:href="#m6ce50a83c0" y="120.636846"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="469.559068" xlink:href="#m6ce50a83c0" y="120.693068"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="471.598355" xlink:href="#m6ce50a83c0" y="121.087502"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="473.637643" xlink:href="#m6ce50a83c0" y="121.340968"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="475.67693" xlink:href="#m6ce50a83c0" y="121.605027"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="477.716217" xlink:href="#m6ce50a83c0" y="121.713755"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="479.755505" xlink:href="#m6ce50a83c0" y="121.748803"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="481.794792" xlink:href="#m6ce50a83c0" y="121.800769"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="483.834079" xlink:href="#m6ce50a83c0" y="121.898552"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="485.873367" xlink:href="#m6ce50a83c0" y="122.008536"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="487.912654" xlink:href="#m6ce50a83c0" y="122.106288"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="489.951942" xlink:href="#m6ce50a83c0" y="122.1421"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="491.991229" xlink:href="#m6ce50a83c0" y="122.159138"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="494.030516" xlink:href="#m6ce50a83c0" y="122.416034"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="496.069804" xlink:href="#m6ce50a83c0" y="122.416034"/>
     <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="498.109091" xlink:href="#m6ce50a83c0" y="122.533153"/>
    </g>
   </g>
   <g id="patch_3">
    <path d="M 72 378 
L 72 51.84 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="patch_4">
    <path d="M 518.4 378 
L 518.4 51.84 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="patch_5">
    <path d="M 72 378 
L 518.4 378 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="patch_6">
    <path d="M 72 51.84 
L 518.4 51.84 
" style="fill:none;stroke:#000000;stroke-linecap:square;stroke-linejoin:miter;stroke-width:0.8;"/>
   </g>
   <g id="legend_1">
    <g id="patch_7">
     <path d="M 82.5 370.5 
L 176.446875 370.5 
Q 179.446875 370.5 179.446875 367.5 
L 179.446875 280.93125 
Q 179.446875 277.93125 176.446875 277.93125 
L 82.5 277.93125 
Q 79.5 277.93125 79.5 280.93125 
L 79.5 367.5 
Q 79.5 370.5 82.5 370.5 
z
" style="fill:#ffffff;opacity:0.8;stroke:#cccccc;stroke-linejoin:miter;"/>
    </g>
    <g id="line2d_22">
     <path d="M 85.5 290.078906 
L 115.5 290.078906 
" style="fill:none;stroke:#0000ff;stroke-linecap:square;stroke-width:3;"/>
    </g>
    <g id="line2d_23"/>
    <g id="text_20">
     <!-- p=0.2 -->
     <g transform="translate(127.5 295.328906)scale(0.15 -0.15)">
      <defs>
       <path d="M 1159 525 
L 1159 -1331 
L 581 -1331 
L 581 3500 
L 1159 3500 
L 1159 2969 
Q 1341 3281 1617 3432 
Q 1894 3584 2278 3584 
Q 2916 3584 3314 3078 
Q 3713 2572 3713 1747 
Q 3713 922 3314 415 
Q 2916 -91 2278 -91 
Q 1894 -91 1617 61 
Q 1341 213 1159 525 
z
M 3116 1747 
Q 3116 2381 2855 2742 
Q 2594 3103 2138 3103 
Q 1681 3103 1420 2742 
Q 1159 2381 1159 1747 
Q 1159 1113 1420 752 
Q 1681 391 2138 391 
Q 2594 391 2855 752 
Q 3116 1113 3116 1747 
z
" id="DejaVuSans-70" transform="scale(0.015625)"/>
       <path d="M 678 2906 
L 4684 2906 
L 4684 2381 
L 678 2381 
L 678 2906 
z
M 678 1631 
L 4684 1631 
L 4684 1100 
L 678 1100 
L 678 1631 
z
" id="DejaVuSans-3d" transform="scale(0.015625)"/>
       <path d="M 684 794 
L 1344 794 
L 1344 0 
L 684 0 
L 684 794 
z
" id="DejaVuSans-2e" transform="scale(0.015625)"/>
      </defs>
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-30"/>
      <use x="210.888672" xlink:href="#DejaVuSans-2e"/>
      <use x="242.675781" xlink:href="#DejaVuSans-32"/>
     </g>
    </g>
    <g id="line2d_24">
     <path d="M 85.5 312.096094 
L 115.5 312.096094 
" style="fill:none;stroke:#008000;stroke-dasharray:11.1,4.8;stroke-dashoffset:0;stroke-width:3;"/>
    </g>
    <g id="line2d_25"/>
    <g id="text_21">
     <!-- p=0.4 -->
     <g transform="translate(127.5 317.346094)scale(0.15 -0.15)">
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-30"/>
      <use x="210.888672" xlink:href="#DejaVuSans-2e"/>
      <use x="242.675781" xlink:href="#DejaVuSans-34"/>
     </g>
    </g>
    <g id="line2d_26">
     <path d="M 85.5 334.113281 
L 115.5 334.113281 
" style="fill:none;stroke:#ff0000;stroke-dasharray:3,4.95;stroke-dashoffset:0;stroke-width:3;"/>
    </g>
    <g id="line2d_27"/>
    <g id="text_22">
     <!-- p=0.6 -->
     <g transform="translate(127.5 339.363281)scale(0.15 -0.15)">
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-30"/>
      <use x="210.888672" xlink:href="#DejaVuSans-2e"/>
      <use x="242.675781" xlink:href="#DejaVuSans-36"/>
     </g>
    </g>
    <g id="line2d_28">
     <path d="M 85.5 356.130469 
L 115.5 356.130469 
" style="fill:none;stroke:#1f77b4;stroke-dasharray:19.2,4.8,3,4.8;stroke-dashoffset:0;stroke-width:3;"/>
    </g>
    <g id="line2d_29">
     <g>
      <use style="fill:#1f77b4;stroke:#1f77b4;stroke-linejoin:miter;" x="100.5" xlink:href="#m6ce50a83c0" y="356.130469"/>
     </g>
    </g>
    <g id="text_23">
     <!-- p=1 -->
     <g transform="translate(127.5 361.380469)scale(0.15 -0.15)">
      <use xlink:href="#DejaVuSans-70"/>
      <use x="63.476562" xlink:href="#DejaVuSans-3d"/>
      <use x="147.265625" xlink:href="#DejaVuSans-31"/>
     </g>
    </g>
   </g>
  </g>
 </g>
 <defs>
  <clipPath id="pcfdc21f5b5">
   <rect height="326.16" width="446.4" x="72" y="51.84"/>
  </clipPath>
 </defs>
</svg>

